Are we there yet? An Industrial Viewpoint on Provenance-based Endpoint Detection and Response Tools

Provenance-Based Endpoint Detection and Response (P-EDR) systems are deemed crucial for future APT defenses. Despite the fact that numerous new techniques to improve P-EDR systems have been proposed in academia, it is still unclear whether the industry will adopt P-EDR systems and what improvements the industry desires for P-EDR systems. To this end, we conduct the first set of systematic studies on the effectiveness and the limitations of P-EDR systems. Our study consists of four components: a one-to-one interview, an online questionnaire study, a survey of the relevant literature, and a systematic measurement study. Our research indicates that all industry experts consider P-EDR systems to be more effective than conventional Endpoint Detection and Response (EDR) systems. However, industry experts are concerned about the operating cost of P-EDR systems. In addition, our research reveals three significant gaps between academia and industry: (1) overlooking client-side overhead; (2) imbalanced alarm triage cost and interpretation cost; and (3) excessive server-side memory consumption. This paper's findings provide objective data on the effectiveness of P-EDR systems and how much improvements are needed to adopt P-EDR systems in industry.

==> tex/backup.tex <==
% five security managers from consumers of \ac{edr} products and five tech managers from the developers, respectively. The managers interviewed are from ten companies, including world-level IT companies and security vendors.  They have 10-15 years of experience in the security industry and lead teams with 20-30 full-time engineers.
% The detailed information of the managers is in Table~\ref{tab:Interview_backgroud}.  
%Bytedance and Sangfor each had two interviewees. However, the two interviewees in the same company are from different departments. Note that both Sangfor and Bytedance are giant IT companies with more than XXX employees. Although they both have departments which build \ac{edr} products, other departments are not necessarily the their consumers. 
% The managers have 10-15 years of experience in security industry and lead teams with 20-30 members.
% The detailed information of the managers is in Table~\ref{tab:Interview_backgroud}. 


% \begin{table*}[]
% \centering
%     \caption{The detailed information of the Interviewees}
%         \resizebox{0.99\textwidth}{!}{
% \begin{tabular}{|c|c|c|c|c|c|c|}
% \hline
% ID  & Company Name                   & Industry Area  & Job Title                 & Years of Exp. & Team Size & Team Type     \\ \hline
% E1  & ByteDance                      & Technology  & Head of Server Security & 6             & 20$\sim$25         & EDR Consumer  \\ \hline
% E2  & MeiTuan       & Technology       & Cloud Workload Security Leader               & 5            & 20$\sim$25         & EDR Consumer  \\ \hline
% E3  & Peking University             & Education     & Director of Network Security Office & 19             & 10$\sim$15         & EDR Consumer  \\ \hline
% E4  & S.F. Express                  & Express & Endpoint Security Manager      & 10             & 20$\sim$25         & EDR Consumer  \\ \hline
% E5  & FiberHome                     & Manufacturing           & Endpoint Security Manager & 8             & 5$\sim$10         & EDR Consumer  \\ \hline
% E6 & Tencent SEC  & Security       & Director of EDR             & 10    & 10$\sim$15         & EDR Developer \\ \hline
% E7  & TrendMicro & Security & Detection Engine Architect of EDR          & 9             & 20$\sim$25         & EDR Developer \\ \hline
% E8  & Sangfor & Security     & Director of Workload Protection Product      & 8             & 65$\sim$70         & EDR Developer \\ \hline
% E9  & Rising   & Security       & EDR Architect          & 21             & 50$\sim$55        & EDR Developer \\ \hline

% E10  & NSFOCUS   & Security     & EDR Product Manager          & 9             & 30$\sim$35         & EDR Developer \\ \hline

% \end{tabular}}
%     \label{tab:Interview_backgroud}

% \end{table*}



% is the minimum estimated value of the managers and the higher bound is the maximum  

% of quantitative reference values, we divide it into five levels plus a "I don't know" as six options according to the range given by the experts. The values of the five options are estimated based on the answers of the technique managers. 

% For example, the reference value range of Network is 1 - 100 MB/day/host, so we set the six options as: A. 1 - 25, B. 25 - 50, C. 50 - 75, D. 75 - 100, E. more than 100, F. I don't know. Level One to Level Five sorted by increasingly loose restrictions.


\eat{
需要说明的是，accuracy的区间太小，不以此为划分；graph size很多人没用过，问卷受访者也很难拿到准确值；
超过90\%的人选项都在interview experts给的范围内，反向验证了专家给的范围的合理性。
每个指标的subrange的分布不同；
1.比较集中的指标，大家比较一致的认可
client side overhead，50-100MB/host
2.集中在多个subrange的指标，大家大致同意
区别不大的是network，1-25与26-50差不多
3.分散在三个以上subrange
意见不是非常一致


discussion
使用interview中的range作为参考，来划分区间是否合理？
questionaire可能存在与interview不一致的看法
questionaire中有些结果比较接近，是否有必要细分到这个粒度；还是说，从新设计问卷，通过受访者来印证采访的结果是正确的。
}








% Interestingly, we observe that existing \ac{edr} systems fail to balance the investigation cost and the triage cost.
% For the \ac{edr} systems that meet the experts' expectations of investigation cost (<10-100 nodes in provenance graphs), they fail to achieve satisfying triage cost. For instance, in Table~\ref{tab:literature}, MORSE and RapSheet can roughly meet the requirement of investigation cost. However, their precision is lower than 0.5, indicating a high number of alerts per host per day in practice. In Table~\ref{tab:graph-size}, HOLMES and ProvDetecor also have concise provenance graphs that meet the expectations of experts. Yet, these two approaches need to reduce the number of alerts by magnitudes. On the flip side, the triage cost of UNICORN is satisfying. However, UNICORN generates too coarse-grained provenance graphs that are three to four magnitude larger than the expectations of experts. 

% With more investigations, we find there is a trade-off between the investigation cost and the triage cost. Assume that the volume of provenance data is fixed. Generating larger provenance graphs can reduce the total number of alerts, leading to fewer number of alerts per host per day. For instance, assume a monitored host generates 10M nodes in a single huge provenance graph. A coarse-grained \ac{pedr} system, such as UNICORN, only generates one alert that covers the whole provenance graph. Thus, its average number of alerts per host per day is low. On the contrary, fine-grained approaches, such as ProvDetecor, generates hundreds of alerts, each covering a subset of the whole provenance graph. Therefore, fine-grained approaches have a higher triage cost. Overall, we identify how to balance the triage cost and investigation cost as a challenge for provenance techniques.


% \begin{tcolorbox}[title=Alert Triage Cost, left=2pt, right=2pt, top=2pt, bottom=2pt]
% Most \ac{pedr} systems still need to reduce the number of alerts per monitored host per day by magnitudes to meet the expectation of industrial experts. 
% \end{tcolorbox}



% \section{Key Takeaway Point}
% The key takeaway point of our interview is that
% the primary decision factor for the experts to adopt an 
% \ac{edr}/\ac{pedr} solution is the \textit{COST} instead of the 
% accuracy. This conclusion is beyond our expectations 
% because the most important metric evaluated in 
% academic papers is accuracy~\cite{}. However, 
% experts from the industry surprisingly disregard the 
% accuracy of \ac{edr} productions.  Eight out of the 
% ten experts do not even consider detection accuracy 
% among their key decision factors of choosing \ac{edr} 
% solutions. The only two experts (E2 and E3)  
% consider detection accuracy as a decision factor. However, they rank it after other decision factors and think it is optional. For instance, as mentioned by E5: "The \ac{edr} we are using now is not the most effective one in detecting attacks, but the most cost-effective. We had multiple choices which had much higher detection accuracy, but they are too expensive to use." 

% \dingli{The reasons should be confirmed}After more discussion with the ten experts, we find  that experts prioritize cost over detection accuracy because 
% \dongfeng{
% there are two prerequisites for \ac{edr} detection attacks: 1). It cannot affect the normal running of the original business on the client-side, otherwise \ac{edr} will not be allowed to install and run; For example, the manager E4 says: "It is our primary goal to ensure the stable operation of the express online business. We will do a performance test for 1-2 months before the installation and upgrade of \ac{edr}. If the business is interrupted due to the occupation of \ac{edr} resources in the production environment, not only \ac{edr} will be removed immediately, but the entire security team will also be punished." 2). The detection result can be confirmed by the analyst, otherwise EDR cannot be used normally. As mentoined by E1: "If the number of \ac{edr} alerts exceeds the processing capacity of analysts, it will gradually become a decoration and cannot play a security role because no one wants to use it."
% }
%they are under the pressure of a frugal budget. For example, the manager EX says: "Our department is under a very tight budget limit. We want our \ac{edr} to be cheap enough. After all, the chance of getting a serious attack is not very high. But a high cost (for the \ac{edr} system) can immediately lead to a NO."


%Companies consider endpoint security as a balance between potential loss of attacks and the cost of having an \ac{edr} solution~\cite{}. Thus, the budget for the security department is limited because the chance of having a successful cyber-attack that leads to significant monetary loss is low~\cite{}. In fact, the ten experts all mentioned that their departments are struggling with the tight budget, so they cannot accept an expensive \ac{edr} solution, regardless of its detection accuracy. \dingli{@dongfeng, you may want to change the next sentence for real feedback from the interview}For example, the manager EX says: "Our department is under a very tight budget limit. We want our \ac{edr} to be cheap enough. After all, the chance of getting a serious attack is not very high. But a high cost (for the \ac{edr} system) can immediately lead to a NO."  

% According to the experts, there are two categories of cost that concern them, as listed in Table~\ref{tab:FactorDefinitions0}. The first category is the \textit{machine cost}, including the client-side overhead, network cost, storage cost, and server-side computing cost.  The second category is the \textit{labor cost}, which represents how many man-hours should be used to maintain the \ac{edr} system. The labor cost includes two aspects: alert triage cost and interpretation cost. Particularly, the experts ranked the client-side overhead as the MOST important decision factor and the triage cost as the second most important one. Besides, the experts also mark the server-side computing cost and the interpretation cost as must-meet requirements for an \ac{edr}/\ac{pedr} system.  


% Specifically, client-side overhead is how much  an \ac{edr} system slows down the protected hosts, network cost is the bandwidth occupied by transmitting system logs to the server, storage cost is hard-disk used to store the system logs, and server-side computation cost is the memory cost on the server to process the collected logs. The second category is the \textit{labor cost}, which represents how many man-hours should be used to maintain the \ac{edr} system. The labor cost includes two aspects: alert triage cost and interpretation cost. Alert triage cost is the man-hour required to triage the detection results, and interpretation cost is the man-hour required to interpret the detection results. We summarize each aspect of machine and labor cost in Table~\ref{tab:FactorDefinitions0}.



% \textbf{Accuracy Under Cost Constraints.}
% Note that we do not conclude that accuracy is not important for \ac{edr}/\ac{pedr} systems. In fact, we strongly believe that achieving high accuracy is one of the fundamental goals for an \ac{edr}/\ac{pedr} system. Our conclusion is that accuracy should not be considered alone. \textbf{Instead, we should balance the accuracy and cost of an \ac{edr} system.}



% In fact, none of our participants have denied the importance of detection accuracy. They just consider accuracy as a part of the labor cost. More specifically, our participants consider improving the accuracy of a \ac{pedr} as a way to reduce the cost of triaging false alerts and fixing successful attacks. By considering accuracy as a part of labor cost, it is possible for security managers to quantitatively balance the cost and performance of a \ac{pedr} system. 
% \begin{tcolorbox}[title=Takeaway Point, left=2pt, right=2pt, top=2pt, bottom=2pt]
% Cost is the primary decision factor for the industry to choose an \ac{edr}/\ac{pedr} system. Developers of \ac{edr}/\ac{pedr} systems should carefully balance the cost and the accuracy. 
% \end{tcolorbox}
% agree that an accurate \ac{pedr} system can reduce their alert triage cost by having fewer false positives. 


% Exceeding our expectations, as the most concerned factor in academic research, only two experts (E2, E3) considered the effectiveness to be an important factor and not necessary. 
% Other experts agree that effectiveness need continuous construction rather than overnight, and related issues can be quickly resolved by upgrading security capabilities, so it is not a key factor. For example, E6 says ``when \ac{edr} has false positives and false negatives, we can solve the problem well by upgrading the ruleset or security model, and never remove \ac{edr} because of this.''
% In the process of using \ac{edr} to combat attacks, analysts can manually confirm true positives and false positives from the alarms, but due to the lack of ground truth, false negatives cannot be identified and recalls cannot be calculated. Therefore, in terms of the metrics, both E2 and E3 agree to use precision to measure effectiveness.


  

% shows the complete workflow of participants using EDR to detect attacks and related seven key factors. The workflow includes four parts: data collection, detection, investigation, and validation and the dotted boxes indicate steps that are not necessarily used in the \ac{edr}.
% The key factors considered by the participants are divided into seven factors in three aspects: \textit{machine cost}, \textit{labor cost} and \textit{performance}. Among them, machine cost refers to the cost of machine resources occupied by \ac{edr} in the workflow of detecting attacks, including \textit{factor 1 network}, \textit{factor 2 storage} and \textit{factor 3 computing}. Labor cost refers to the cost for analysts to manually validate alarms or investigation graphs, including \textit{factor 4 graph size}, \textit{factor 5 semantic gap}, and \textit{factor 6 validation amount};
% The performance refers to the performance of \ac{edr} detection, that is, \textit{factor 7 effectiveness}. We summarize the detailed definitions of the seven factors in Table~\ref{tab:FactorDefinitions}.
% In addition to the above seven factors, the participants also mentioned factors in product design and engineering such as stability, compatibility, and self-protection. However, these factors have nothing to do with whether to use the provenance analysis techniques, so they are out of the scope of the discussion.
\eat{
图x展示了受访者使用EDR检测攻击的完整工作流程以及相关关键因素。流程包括数据采集，检测，溯源，人工验证四个步骤，其中虚线框表示EDR中不一定包含的步骤。受访者考虑的关键因素分为机器检测成本，人工验证成本和检测效果三个方面七个因素。其中，机器检测成本指EDR在检测攻击过程中占用的机器资源成本，包括因素1网络传输，因素2存储和因素3计算；
人工验证成本指分析师人工确认告警或调查图正误报的人力成本，包括因素4调查图的大小，因素5告警或调查图研判的语义鸿沟，因素6需要确认的告警数量；
安全效果是指EDR检测的安全效果，即因素7effectiveness。
需要说明的是，受访者也提到了Stability， Compatibility， Self protection等Product design and engineering方面的因素，然而它们与攻击检测的方法无关，因此不在本文讨论的范围内。
}
% We conclude the current \ac{apt} detection routines in \ac{soc} in Figure~\ref{fig:aptroutine}. The methodology of current commercial \ac{edr} is mainly focused on rule matching. Although these methods can detect the occurence of attack, it costs a lot of time during the threat hunting. Our interview shows that the common limitations that commercial \ac{edr} faced are xxx and xxx. The developers have reimplemented several current graph-based detection system, however, they have encountered great difficulty deploying in industrial environments. As said by E1:
% $$xxxx$$

\eat{
表格x展示了所有受访者对EDR日常使用中关键因素的排序，度量方法以及参考值等详细信息。例如，表格第三排第四列中“2，client+server Memory，Client CPU”表示受访者E1认为计算成本是第二重要因素。该因素可以用消耗的客户端内存和CPU来度量，最大参考值分别为100MB/HOST和百分之1。星号表示计算成本指标是EDR产品必须满足的。

总体来说，超出我们的预期，安全专家认为cost是第一重要的因素，而非安全效果。所有10位受访者将机器成本中的计算成本和人力成本中的确认量排在前两位。相反，仅2位专家考虑了安全效果因素，并且都被排在最不重要的因素。原因是EDR检测攻击有两大前提条件：1.不能影响客户端原有业务正常运行，否则EDR不被允许安装运行；2.检测结果能够被分析师确认完，否则EDR无法被正常使用；。例如，E5专家说，我们现在使用的EDR产品并不是检测效果最好的，但是性价比最高的。我们还有很多其他EDR厂商的产品可以选择，但是这些产品需要更多的资源。

E4说，保障快递业务稳定运行是我们首要目标，edr安装和升级前我们都会做长达1-2个月的性能测试。如果在生产环境由于edr资源占用造成业务中断，不仅edr会立刻被淘汰，整个安全部门也会受到惩罚。
E1说，如果edr告警数量超出分析师的处理范围，它将因为没人愿意使用而逐渐成为一个摆设。

}

% \subsection{Detailed Result} 
% In this section, we report the detailed result about key decision factors and limitations of existing \ac{pedr} systems. To better explain the full picture, we also summarize the workflow of existing \ac{pedr} systems in Figure~\ref{fig:EDRworkflow}. The workflow includes four parts: data collection, detection, investigation, and validation, and the dotted boxes indicate steps that are optional in the \ac{edr}. We also put the seven decision factors in Figure~\ref{fig:EDRworkflow} to show how these factors affect different stages of a \ac{pedr} system. 

% We summarize the key decision factors with their corresponding metrics in Table~\ref{tab:InterviewResult}. Each cell inTable~\ref{tab:InterviewResult} is in the form ``rank,  Metric Name: Expected Value, Metric Name: Expected Value...'', where ``rank'' is the rank of importance of the corresponding decision factor of each interviewee. ``Metric Name'' is the name of the metric that the interviewee adopts to evaluate the corresponding key decision factor. We may put an * symbol beside the metric name to indicate the metric is a must-meet condition. ``Expected Value'' represents the expected value of the metric of a key decision factor of an interviewee. If a decision factor has multiple metrics, we enumerate them all. For example, ``3,AveMem*: 30MB/host'' in row E1 and column ``Computing'' means E1 ranked computing cost as the third most important decision factor. He would use the average memory consumption (AveMem) as the concrete metric to measure the computing cost, and he expected the memory consumption to be 30MB per monitored host. The * symbol means the interviewee thinks AveMem must meet his expectation before he can accept a \ac{pedr} system. 

% shows the detailed results of participants on interview questions I2 and I3. For example, "2, Memory*: 100MB/host, CPU*:5\%" in the fifth column of the third row of the table indicates that participants E1 considers computing cost on the client side to be the second most important factor. This factor can be measured by the consumed client memory and CPU, and the maximum reference values are 100MB/host and 1\% respectively. The symbol "*" indicates that this factor must be met by \ac{edr} systems.

% In general, beyond our expectation, we find that the top key decision factor for the managers is  the cost instead of the performance(\ie accuracy). All ten managers put computing(Client) cost in machine cost and validation amount in labor cost in the top two places of \ac{edr} systems. On the flip side, only two experts(E2, E3) rank the effectiveness factor as the least important factor, while other experts even ignore this factor. The rationale is that there are two prerequisites for \ac{edr} detection attacks: 1. It cannot affect the normal running of the original business on the client side, otherwise \ac{edr} will not be allowed to install and run; 2. The detection result can be confirmed by the analyst, otherwise EDR cannot be used normally. As said by E5: "The \ac{edr} we are using now is not the best detection effect, but the most cost-effective. We had multiple choices which had much higher detection accuracy, but they needed too much resources."
%The rationale is that, in most use cases of \ac{edr} systems, security is in fact a trade-off between the expected loss of potential data breaches and the cost to maintain an \ac{edr} system. For instance, the manager from XXX says "when we choose our current \ac{edr} product simply because it is cheap to use. We had multiple choices which had much higher detection accuracy, but they needed too much resources." In practice, since people tends to under-estimate the potential loss of data breaches~\cite{}, they are reluctant to invest security solutions~\cite{}. In fact, XX out of the five consumers of \ac{edr} systems said that their team faced difficulties in asking for budget. Therefore, it is their top concern to reduce the cost of \ac{edr} systems. Particularly, the managers concern two types of cost of an EDR system: the machine cost and the labor cost. 

\eat{
Computing Cost
所有专家都认为计算成本是机器成本中最重要且必需的因素。超过50\%的专家认为网络（E5-E10）与存储成本(E3，E5-10)也是需要考虑的关键但非必需因素。CPU与内存的成本远远高于网络带宽和硬盘价格，因此计算成本是机器成本中最重要因素。网络与存储成本在安全预算中占比较小，不同的客户按需来安排，因此受访者认为它们是非必须因素。

关于如何衡量三个因素，所有的受访者都同意使用平均内存，平均CPU和平均网络传输量来衡量计算和网络成本。其中，运行在受监控主机上的代理与原有业务共用CPU，会直接影响业务的稳定性，因此客户端成本还需要衡量平均CPU。存储成本方面，E3采用集群硬盘空间占比，而E6，E7采用数据缓存天数。然而，由于不同客户的集群主机数量不同，缓存天数要求也不同，这两种指标难以统一衡量比较。通过回访确认，E3，E6，E7也认同采用平均硬盘占用量来衡量存储成本。
专家们都期望EDR尽可能少的消耗机器资源。例如，E5说，我们用于安全业务的机器资源不能超过总集群5\%。我们集群中有2w台主机，如果需要再去花费2000台主机来保护他们是无法接受的。
所有受访者为度量指标给出了自己的参考值。其中，E6-10表示，虽然网络与存储成本不同客户成本不同，他们还是给出了大部分客户能够接受的参考值。E9的avenet为1MB/day/host的原因是，所有数据都在agent上面计算，每天只是上传少量的心跳信息到服务端；





}

% More than 50\% of experts think network (E5-E10) and storage cost (E3, E5-10) are also key but unnecessary factors to be considered. 
% The cost of CPU and memory is much higher than the price of network bandwidth and hard disk, so computing cost is the most important factor in machine cost. Network and storage costs account for a relatively small proportion of the security budget, and different customers arrange them according to their needs, so experts consider them to be unnecessary factors.
% With respect to the metrics, all experts agreed to use the average memory (AveMem) and average network transmission volume (AveNet) to measure computing and network costs. 
% In addition, the agent running on the monitored machine shares the CPU with the original business, which will directly affect the stability of the business, so the client computing cost also needs to measure the average CPU (AveCPU).
% In terms of storage cost measurement, E3 uses the proportion of cluster hard disk space, while E6 and E7 use the number of days of data cache. However, since different customers have different numbers of cluster machines and different data cache days requirements, it is difficult to measure and compare these two indicators uniformly. It was confirmed through a return visit that E3, E6, and E7 also agreed to use the average hard disk usage (AveDisk) to measure storage costs.
% All experts expect EDR to consume as little machine resources as possible. For example, E5 says that we cannot use more than 5\% of the total cluster's machine resources for security operations. We have 20,000 hosts in our cluster, and it is unacceptable to spend another 1,000 hosts to protect them. 
% All experts gave their own reference values for the metrics. Among them, E6-10 said that although the cost of network and storage varies from customer to customer, they still give a reference value that most customers can accept. The reason why the AveNet of E9 is 1MB/day/host is that all data is calculated on the agent, and only a small amount of heartbeat information is uploaded to the server every day;
%With respect to the machine cost, the managers mentioned three aspects of the machine cost, which are computing cost, network cost, and storage cost. 
%Specifically, the managers expect EDR systems to consume little memory on the monitored machines and occupy mediocre bandwidth and storage in the centralized \ac{soc}. 
%With respect to the metrics, all managers agree to use the average memory cost of each agents on monitored machines(AveMem), the average amount of data transmitted over network per monitored host per day (AveNet), and the average disk occupation per host per day (AveDisk) as metrics for the three aspects of costs. We summarize the detailed definitions of the three metrics in Table~XXX.

\eat{
Labor Cost
8位专家认为研判量是人工成本中最重要且必须的因素。此外，支持告警调查图的EDR专家（E1,E2,E6,E7）均认为调查图大小是也是重要且必须的因素。
仅仅E2一位专家考虑了告警语义鸿沟因素，并且认为是非必须因素。
确保研判量在客户分析师可处理的范围以内，是EDR能够被使用的前提条件，因此研判量是人工成本中最重要因素。例如，E5说，我们的分析师每天最多处理400告警，超过部分就会被忽略，意味着会面临告警疲劳问题。告警调查图大小超过一定规模后，会导致分析师陷入调查疲劳，因此对于支持告警调查图的EDR来说，告警调查图大小是重要且必须因素。通过对除E2外专家回访确认，他们认为分析师的告警语义翻译能力与其经验有关，大部分成熟分析师较少碰到这个问题。通常经验不足的新人分析师会面临告警语义鸿沟问题，也可以通过快速培训来缓解这个问题。

关于如何衡量三个因素，所有的受访者都同意使用平均告警量、图节点数量以及语义级别来衡量研判量、图大小以及语义鸿沟三个因素，并且分别给出了自己的参考值。
可以看到，不同专家给出的平均告警量参考值波动幅度很大（0.001~0.1/day/host）。所有的专家都说他们的分析师人数固定，因此每天能处理的告警数量也是固定的。不同客户可处理告警量的差异远小于受保护的机器数量差异，导致了如此大的波动幅度。例如，E5说，他们公司2个分析师每天只能处理400个告警，要负责处理2w台主机告警，所以他们的平均告警量为0.02alarms/day/host（400/20000）。E7说使用他们产品的客户通常仅有1个分析师，每天可以处理100条，负责处理约1000台主机告警，因此他们的平均告警量为0.1alarms/day/host（100/1000）. 此外，由于E1-2主机规模在100w以上，E4，E5主机规模在1-10w，E6-10客户集群大部分在1000左右，可以看到，随着主机规模的增加，客户对告警疲劳的容忍度越低，要求平均告警量值越小。


研判成本与告警总量正相关。
Eight out of the ten experts mentioned that their team or customer has a fixed number of analysts to investigate the alarms and thus they can only process a fixed number of alarms per day. 由于不同公司需要保护的主机数量差别较大，为了方便统一量化，受访者选择使用平均告警数量来衡量成本。


}


% \subsubsection{Labor Cost}
% \label{sec:laborcost}
% According to our participants, the most important decision factor for the labor cost is the alarm triage cost. Particularly, eight out of ten participants mark the triage cost as a must-meet requirement. Two participants ranked the triage cost as the MOST important decision factor, and the other six ranked it as the SECOND most important decision factor. 

% With respect to the metric for the triage cost, the participants agreed on using the average number of alarms per monitored host per day to measure the triage cost. 
% The rationale is that the triage cost is positively correlated with the number of alarms. Eight out of the ten experts mentioned that their team or customer has a fixed number of analysts to investigate the alarms and thus they can only process a fixed number of alarms per day. The number of hosts that companies need to protect varies widely, so the participants choose to use the average number of alarms as the metric for the triage cost.

%This is beyond our expectations because it is the accuracy that fundamentally determines the triage cost, but the average number of alerts is a very imprecise metric for accuracy. However, after having more discussions with our participants, we realize that the average number of alerts is a more practical metric for the triage cost.

%\dingli{These reasons may be improved}The reason that the participants choose to use the average number of alerts as the metric for the triage cost is three-fold. First, it is hard to get the real accuracy for a \ac{pedr} system. As mentioned by EX: ``the accuracy numbers for \ac{edr} systems are all based on simulated environments, which can hardly represent our realistic situations.'' Second, the average number of alerts is, in fact, a good-enough approximation of the precision. In real enterprise environments, it is rare to encounter attacks. Therefore, most of the  alerts of an \ac{edr} system are false alerts. So, the average number of alerts can often be approximately considered as the average number of false alerts on a fully benign dataset. Third, it is straightforward to get the average number of alerts. Thus, users can quickly evaluate the triage cost of a \ac{pedr} system.

% The participants are particularly sensitive to the average number of alarms. The highest number is 0.1 per monitored host per day. E1 and E2 gave the lowest value, which was 0.001 per monitored host per day. The reason is that the security operation teams in the industry are often limited in personnel. Thus, they can only process a fixed number of alarms per day. For example, E5 said that there are only two analysts in their company that could handle 400 alarms per day. This team is responsible for 20,000 hosts, so they want the average number of alarms to be 0.02 per host per day (400 alarms/20,000 hosts). E7 also said that customers who use their products usually only have one analyst who can handle 100 alarms per day and are responsible for about 1,000 hosts, so he expects the average number of alarms to be 0.1 per host per day (100 alarms/1000 hosts). 



% In addition, Since the scale of E1-2 hosts is above one million, the scale of E4 and E5 hosts is 10,000~100000, and most of the E6-10 customer clusters are around 1000, it can be seen that as the scale of hosts increases, customers are more tolerant of alarm fatigue.

% Besides the triage cost, the four participants who are either using provenance analysis techniques or developing provenance-analysis-based solutions also mart the interpretation cost as a must-meet requirement. They agreed to use the average number of nodes of provenance graphs of alarms as the metric for the interpretation cost. The reason is that \ac{pedr} systems generate a provenance graph for each alarm to track its context. Thus, the size of the provenance graphs determines the workload for the security team to interpret the provenance graphs. Particularly, the participants expect the average number of nodes of provenance graphs between 10 to 100.   

% \begin{tcolorbox}[title=Conclusion for labor cost, left=2pt, right=2pt, top=2pt, bottom=2pt]
% Managers in the industry are sensitive to the alarm fatigue problem. Thus, the triage cost is the most important decision factor in labor cost. Besides, the investigation cost is also a must-meet requirement. 
% \end{tcolorbox}

% In other words, our participants expect an \ac{pedr} system to generate at most one alert for 10-100 monitored host per day. 
 
% For labor cost, the key concern of the experts is validation amount. In addition, those experts (E1, E2, E6, E7) whose \ac{edr} can generate alarm investigation graphs agree that the graph size is also an important and necessary factor. Only one expert (E2) consider semantic gap factor to be important, but not necessary.
% Ensuring that the number of alarms that need to be validated is within the range that analysts can handle is a prerequisite for \ac{edr} to be used. Therefore, validation amount is the most important factor in labor costs.
% All experts concerned that an overly large provenance graph may exhaust their limited labor budget for investigation.
%When the size of the alarm investigation graph exceeds a certain threshold, analysts will fall into investigation fatigue.
% Therefore, for \ac{edr} that supports the alarm investigation graph, graph size is an important and necessary factor. Regarding the semantic gap factor, experts other than E2 agree that an analyst's ability to translate alarm semantics is related to his experience, and most mature analysts seldom encounter this problem. Usually inexperienced novice analysts will face the problem of semantic gap, which can also be alleviated by quick training.
% With respect to the metrics, all experts agree to use the average number of alarms (AveAlarm), the number of graph nodes, and the semantic level as metrics for the three aspects of costs and give their own reference values respectively.
% It can be seen that the AveAlarm reference value given by different experts fluctuates greatly (0.001-0.1/day/host). 
% Eight out of the ten experts mentioned that their team or customer has a fixed number of analysts to investigate the alarms and thus they can only process a fixed number of alarms per day. The difference in the amount of alarms that can be handled by different customers is much smaller than the difference in the number of protected machines, resulting in such a large fluctuation. For example, E5 said that two analysts in their company can only handle 400 alarms per day, and they are responsible for 20,000 hosts, so their AveAlarm is 0.02 alarms/day/host (400 alarms/20,000 hosts). E7 said that customers who use their products usually only have 1 analyst, who can handle 100 alarms per day and are responsible for about 1,000 hosts, so their AveAlarm is 0.1 alarms/day/host (100 alarms/1000 hosts). In addition, Since the scale of E1-2 hosts is above 1 million, the scale of E4 and E5 hosts is 10,000~100000, and most of the E6-10 customer clusters are around 1000, it can be seen that as the scale of hosts increases, customers are more tolerant of alarm fatigue.

%For labor cost, the key concern of the managers is the number of engineers required to effectively use an \ac{edr} system. In this sense, the managers agreed that the detection accuracy of an \ac{edr} system is important. After all, an accurate \ac{edr} system can reduce the labor cost to investigate and triage alerts of an \ac{edr} system. However, different from our original expectation, the managers did not pursue a perfect accuracy, but instead, an enough accuracy under a fixed constraint of labor cost. Particularly, X out of the five managers of \ac{edr} consumers mentioned that their team has a fixed number of engineers to investigate the alerts and thus their team can only process a fixed number of alerts per day. Therefore, these managers only concern the accuracy of an \ac{edr} system under the condition that it does not generate too many alerts that the team cannot process. The five managers of the developer of \ac{edr} system agreed with the consumers and mentioned that their customers also have similar concerns. 


\eat{
超出我们的预期，作为学术研究中最关心的因素，只有两个专家（E2，E3）认为安全效果为一个重要的因素，而且并不是必需的。其他专家均认为，安全效果是一个持续建设的过程，可以通过升级安全能力快速提升解决，所以不是关键考虑因素。例如，E6说，当EDR发生误报漏报时，我们通过升级规则库或者安全模型很好的解决问题，从来不会因此下架EDR。
在使用EDR对抗攻击过程中，分析师可以从告警中人工确认出true positive，false negative，但由于缺乏ground truth，无法识别false negative，无法计算recall。因此，安全效果度量方面，E2，E3均同意使用precision来衡量安全效果。

}


%To be more specifically, the the most decisive metric that the managers concern is the number of alerts generated by an \ac{edr} system per day. All of the ten managers mentioned that this is the first metric they consider while choosing or developing an \ac{edr} system, without considering the accuracy. Particularly, the manager from XXX mentioned ``while accuracy is definitely important, it is too costly for us to get the precise number. The number of alerts is more straightforward to measure and interpret in practice.''  

%The second important metric for the labor cost is the false positive rate. All managers mentioned that they do not want an \ac{edr} system to generate too many false positives that waste their labor cost. Surprisingly, on the flip side, the managers do not pay much attention to negatives. Only X out of the five consumers and X out the five developers have mentioned false negative rate in their interviewee, without emphasize. The primary reason is that it is hard to precisely measure the true false negative rate. For instance, one manager says ``Of course we want it(the \ac{edr} system) to detect attacks, but it is really for us to know how good it is. Besides, we are not expecting it to make our system 100\% secure.''

\eat{
limitations and Dream EDR
表格x中展示了受访者认为的现有EDR不足。可以看到，性能影响，误报和未知攻击是专家们广泛认同的不足点。所有的专家都认为现有的EDR产品性能消耗还是对业务产生了影响，还有改善的空间。70\%的专家认为现有EDR产品在大规模集群上依然存在比较严重的告警疲劳问题。7位专家认为采用基于规则的检测方法对未知攻击检测效果不足。此外，缺乏响应能力，缺乏上下文导致研判困难以及edr数据采集带来的隐私问题，也被少数几位专家提出来。

溯源图技术
4位专家提到他们的产品中使用溯源图进行攻击溯源，即以告警事件为起点，通过因果分析回溯出一个有限范围的溯源图方便人工调查。其他复杂的溯源图计算，例如基于溯源图的攻击检测、攻击图关联等，并没有在EDR产品中应用。
所有的专家都同意溯源图分析技术能够提升攻击检测效果，并且有兴趣在产品中使用。例如，E8表示，他们曾尝试用溯源图检测攻击。然而，仅一台主机溯源图数据就需要800MB内存来检测攻击，一个客户有1200台主机，实验服务器仅跑了40台主机数据就内存不足，公司找不到900+G服务器来检测攻击；尽管如此，我们依然希望找到可行的方法。


E2,基于规则的检测方法依赖于安全专家提取规则，因此对新出现的未知攻击检测存在滞后性。我们只能通过提升规则更新速度来缓解滞后性，但是无法彻底解决这个问题。

E3,由于担心edr采集数据侵犯个人或公司隐私，很多客户对edr的安装和使用持有怀疑甚至反对的态度。
专家们不考虑recall和accuracy是因为在实际场景下，缺乏groundtruth，分析师无法确认false negatives，因此无法系统性衡量EDR的recall和accuracy。
}


% \subsubsection{Accuracy}
% Only two experts(E2 and E3) mentioned that they consider accuracy as one of the optional decision factors for choosing \ac{edr}/\ac{pedr} systems.  
% \dongfeng{
% Other experts agree that effectiveness need continuous construction rather than overnight, and related issues can be quickly resolved by upgrading security capabilities, so it is not a key factor. For example, E6 says ``when \ac{edr} has false positives and false negatives, we can solve the problem well by upgrading the rule set or security model, and never remove \ac{edr} because of this.''
% }
% Particularly, they mentioned that they are interested in the precision of an \ac{edr}/\ac{pedr} system since a system with low precision can generate more false positives that increase the triage cost. 
% \dongfeng{
% Experts do not consider recall and accuracy. The reason is that due to the lack of ground truth, analysts cannot find false negatives and cannot evaluate the recall and accuracy of an \ac{edr}/\ac{pedr} system in practice.
% }
% %The experts do not consider recall because it is impossible for them to systematically evaluate the recall of an \ac{edr}/\ac{pedr} system in practice. 
% However, the experts still think that an \ac{edr}/\ac{pedr} system should be able to detect a large number of attacks. The only thing is that they do not have a way to quantitatively evaluate how well can an \ac{edr}/\ac{pedr} system detect real attacks.  

% \subsubsection{Summary of Limitations}


% We summarize the limitations of \ac{pedr} mentioned by our participants in Table~\ref{tab:Interview_limitations}. All participants complained that the client-side overhead of existing \ac{pedr} systems are too high. Seven participants also mentioned that existing \ac{pedr} systems generate too many false positives. 

% Besides high client-side overhead and false alarm rate, seven out of ten participants also mentioned their concerns about the incomplete rule set of their \ac{edr} and \ac{pedr} system could not detect unknown attacks. 
% \dongfeng{For example, E2 said ``Rule-based detection methods rely on security experts to extract rules, so there is a lag in the detection of emerging unknown attacks. We can only alleviate the lag by increasing the rule update speed, but cannot completely solve this problem.``}
% Overall, all of our participants have mentioned that they are looking for more general learning-based techniques to take the place of their existing rule-based systems.

% Lastly, E3 also mentioned that he is concerned about the privacy risks of the \ac{edr} system he is using. He said: 
% \dongfeng{"Because of the fear that edr data collection may infringe on personal or company privacy, many customers are skeptical or even opposed to the installation and use of \ac{edr}."}

% \begin{tcolorbox}[title=Conclusion for limitations, left=2pt, right=2pt, top=2pt, bottom=2pt]
% Managers agreed that the main limitations of existing \ac{pedr} systems are high client-side overhead and high false positive rate. Besides, they are also worried about the incomplete rule set and privacy issues. 
% \end{tcolorbox}
% Performance impact, false alarm, and unknown attacks are the TOP 3 limitations widely agreed by the experts. All experts agree that the performance consumption of existing \ac{edr} products still has an impact on the original business, and there is still room for improvement. 
% 70\% of the experts mentioned that existing \ac{edr} products still have serious alarm fatigue problems on large-scale clusters, and the rule-based method cannot detect unknown attacks well.
% In addition, limitations such as lack of responsiveness, difficulty in attack investigation due to lack of context, and data privacy concerns posed by \ac{edr} data collection were also raised by a few experts.

% \textbf{Provenance Analysis Techniques.}
% For the questions related to provenance analysis techniques, four experts mentioned that their products use provenance analysis techniques for attack investigation.
% The \ac{edr} takes the alarm event as the starting point, and generates a limited provenance graph through causal analysis for manual confirmation. 
% All experts agree that provenance graph analysis can improve attack detection and are interested in using it in products. 

%X of the managers mentioned that they are using provenance analysis techniques in their current \ac{edr} systems. X of the managers said they use provenance analysis techniques to detect APT attacks while X said they use provenance analysis techniques for attack investigation. For the rest X managers who is not using provenance analysis techniques, they showed strong interests in using these techniques. For instance, one of the manager said ``This(provenance analysis) looks promising, could you share me more information?''. 

%All ten managers agreed that provenance analysis techniques can help investigating attacks. However, they also raised concerns about the size of provenance graph. Remember that one of the top decisive factors of the managers is the labor cost. All managers concerned that an overly large provenance graph may exhaust their limited labor budget for investigation. 

% In our interviews, we summarize the routine of \ac{apt} detection and conclude nine key topics and their corresponding metrics to evaluate. Based on these topics, we design our questionnaire to further investigate the specific needs of the industry for these indicators. 

\eat{
\section{Questionnaire}
Our semi-structured interview has summarized the key points that enterprises are most concerned about. Having these key points, the second phase of our survey is carrying out online questionnaires to get quantitative results based on these key points. We use questionnaire to refine the scope of quantitative factors and select ideal scopes that are commonly accepted by security analysts. We design the questions of questionnaire following the general principals~\cite{inbook} and we will disclose it in the followings.
In order to find right respondents, we use the same method as in the above interview, first find the leader of the \ac{edr} development and use team, and then forward the questionnaire to the team members through the leader. At last we received 34 questionnaire responses.
The participants of our questionnaire have a variety of positions and come from various organizations, with different \ac{apt} combatting experience, as shown in Figure~\ref{fig:participants}. Through the online questionnaire, we have obtained the ideal quantitative requirements for each key points in the actual deployment process in industry, listed in Table~\ref{tab:InterviewResult}.


\noindent\textbf{Questionnaire Design}: 
We design the questionnaire based on the seven key factors, metrics and reference value ranges obtained from expert interviews, as shown in Table~\ref{tab:Questionnaire}. It consists of two aspects: Participants' Background, Quantitative reference value of seven factors.  For each question of quantitative reference values, we divide it into five levels plus a "I don't know" as six options according to the range given by the experts. For example, the reference value range of Network is 1 - 100 MB/day/host, so we set the six options as: A. 1 - 25, B. 25 - 50, C. 50 - 75, D. 75 - 100, E. more than 100, F. I don't know. Level One to Level Five sorted by increasingly loose restrictions.
 
The questions in the questionnaire were confirmed by all the interview experts to avoid question deviation and ensure that the questions could be understood by the participants. The length of the questionnaire can be answered within 10 minutes.


\noindent\textbf{Questionnaire Result}:
First of all, we screened and eliminated 2 abnormal questionnaires through the options of answering time less than 100 seconds and the proportion of unknown answers being higher than 50\%, leaving 32 valid questionnaires.
Figure~\ref{fig:participants} shows the background of participants in the survey. We can find that the participants of our questionnaires include people in various positions in various industries. They are  sophisticated with industrial security and have 4.4 years of the \ac{apt} combatting experience on average. Figure~\ref{fig:questionnaire-results} shows the distribution of options for each question. We choose the one with the largest number of people as the reference value of this key factor. We summerize the results of quantitative reference values of seven factors in Table~\ref{tab:QualitativeResult}.

\begin{table}[]
    \caption{Qualitative Result of Our Survey}
    \begin{tabular}{|ll|}
    \hline
    \multicolumn{1}{|l|}{\textbf{Key Factors}}       & \textbf{Qualitative Result}                   \\ \hline
    % \multicolumn{2}{|l|}{\textbf{Limitations}}                                              \\ \hline
    \multicolumn{1}{|l|}{Network}      &  25 $ \sim $ 50 MB/day/host  \\ \hline
    \multicolumn{1}{|l|}{Storage}             &   70 $ \sim $ 100 MB/day/host           \\ \hline
    \multicolumn{1}{|l|}{Computing}          &   30 $ \sim $ 40 MB/host           \\ \hline
    \multicolumn{1}{|l|}{Client-side Overhead (CPU)}            &                     1  $ \sim $ 3 \%                 \\ \hline
    \multicolumn{1}{|l|}{Client-side Overhead (Memory)}            &                     50  $ \sim $ 100 MB/host                 \\ \hline 
    \multicolumn{1}{|l|}{Interpretation Cost}            &  70$ \sim $ 100   \\ \hline
    \multicolumn{1}{|l|}{Alert Triage Cost}            &            0.05 $ \sim $ 0.1 /alarms/day/host                           \\ \hline
    \multicolumn{1}{|l|}{Accuracy}            &         0.8 $ \sim $ 0.9        \\ \hline
    % \multicolumn{2}{|l|}{\textbf{Provenance Analysis Techniques(PAT)}}                      \\ \hline
    % \multicolumn{1}{|l|}{PAT used in current EDR} & E1, E2, E6, E7                          \\ \hline
    % \multicolumn{1}{|l|}{interested in using PAT} & E1, E2, E3, E4, E5, E6, E7, E8, E9, E10                     \\ \hline
    \end{tabular}
    \label{tab:QualitativeResult}
\end{table}



\begin{figure}[t!]
    \includegraphics[width=0.48\textwidth]{fig/questionnaire-result.pdf}
    \caption{Metric Results of Our Questionnaire Study.}
    \label{fig:questionnaire-results}
\end{figure}



\begin{tcolorbox}[title=Answer to RQ1, left=2pt, right=2pt, top=2pt, bottom=2pt]
We conclude with seven key factors from our survey. It consists of three aspects: machine cost, labor cost, and effectiveness. According to our survey, there are four must-meet conditions: computing, client-side overhead, interpretation cost and alert triage cost.
\end{tcolorbox}



\begin{figure*}[!t]
    \centering
    \subfigure[The Role of Participants.]{
    \includegraphics[width=0.3\textwidth]{fig/questionnaire-role.pdf}
    \label{fig:kvalue}}
    \subfigure[The APT Combatting Experience of Participants]{
    \includegraphics[width=0.3\textwidth]{fig/questionnaire-year.pdf}
    \label{fig:ASGSize}}
    \subfigure[The Type of Organizations Participants Work In]{
    \includegraphics[width=0.3\textwidth]{fig/questionnaire-org.pdf}
    \label{fig:ASGf1}}
    % \\
    % \subfigure[Sliding time window]{
    % \includegraphics[width=0.3\textwidth]{fig/questionnaire-year.pdf}
    % \label{fig:time-window}}
    % \subfigure[Similarity threshold $\tau_s$.]{
    % \includegraphics[width=0.3\textwidth]{fig/questionnaire-year.pdf}
    % \label{fig:similarityThreshold}}
    % \subfigure[Ranking threshold $\tau_d$]{
    % \includegraphics[width=0.3\textwidth]{fig/questionnaire-year.pdf}
    % \label{fig:threshold}}
    % %\vspace{-0.1in}
    \caption{Participants of Our Questionnaire Study.}
    % \vspace{-0.1in}
    \label{fig:participants}
\end{figure*}
}



% there are two categories of cost that concern them, as listed in Table~\ref{tab:FactorDefinitions0}. The first category is the \textit{machine cost}, including the client-side overhead, network cost, storage cost, and server-side computing cost.  The second category is the \textit{labor cost}, which represents how many man-hours should be used to maintain the \ac{edr} system. The labor cost includes two aspects: alarm triage cost and interpretation cost. Particularly, the experts ranked the client-side overhead as the MOST important decision factor and the triage cost as the second most important one. Besides, the experts also mark the server-side computing cost and the interpretation cost as must-meet requirements for an \ac{edr}/\ac{pedr} system. 

% Note that, among the four types of cost,XXX 

% , in which $E(loss)$ is the expected loss and $COST$ is the running cost o
% . In fact, we strongly believe that achieving high accuracy is one of the fundamental goals for an \ac{edr}/\ac{pedr} system. Our conclusion is that accuracy should not be considered alone. \textbf{Instead, we should balance the accuracy and cost of an \ac{edr} system.}

% \dingli{The reasons should be confirmed}After more discussion with the ten experts, we find  that experts prioritize cost over detection accuracy because 
% \dongfeng{
% there are two prerequisites for \ac{edr} detection attacks: 1). It cannot affect the normal running of the original business on the client-side, otherwise \ac{edr} will not be allowed to install and run; For example, the manager E4 says: "It is our primary goal to ensure the stable operation of the express online business. We will do a performance test for 1-2 months before the installation and upgrade of \ac{edr}. If the business is interrupted due to the occupation of \ac{edr} resources in the production environment, not only \ac{edr} will be removed immediately, but the entire security team will also be punished." 2). The detection result can be confirmed by the analyst, otherwise EDR cannot be used normally. As mentoined by E1: "If the number of \ac{edr} alarms exceeds the processing capacity of analysts, it will gradually become a decoration and cannot play a security role because no one wants to use it."
% }


% According to the experts, there are two categories of cost that concern them, as listed in Table~\ref{tab:FactorDefinitions0}. The first category is the \textit{machine cost}, including the client-side overhead, network cost, storage cost, and server-side computing cost.  The second category is the \textit{labor cost}, which represents how many man-hours should be used to maintain the \ac{edr} system. The labor cost includes two aspects: alarm triage cost and interpretation cost. Particularly, the experts ranked the client-side overhead as the MOST important decision factor and the triage cost as the second most important one. Besides, the experts also mark the server-side computing cost and the interpretation cost as must-meet requirements for an \ac{edr}/\ac{pedr} system.  


% \textbf{Accuracy Under Cost Constraints.}
% Note that we do not conclude that accuracy is not important for \ac{edr}/\ac{pedr} systems. In fact, we strongly believe that achieving high accuracy is one of the fundamental goals for an \ac{edr}/\ac{pedr} system. Our conclusion is that accuracy should not be considered alone. \textbf{Instead, we should balance the accuracy and cost of an \ac{edr} system.}



% In fact, none of our interviewees have denied the importance of detection accuracy. They just consider accuracy as a part of the labor cost. More specifically, our interviewees consider improving the accuracy of a \ac{pedr} as a way to reduce the cost of triaging false alarms and fixing successful attacks. By considering accuracy as a part of labor cost, it is possible for security managers to quantitatively balance the cost and performance of a \ac{pedr} system. 

% % \section{Literature Investigation and Measurement Study}
% In this section, we investigate recently published \ac{pedr} systems to check whether they meet whether they can meet the four must-meet requirements(client-side overhead, server-side computing cost, triage cost, and interpretation cost). Besides, we also evaluate whether existing approaches can meet the three optional requirements(network cost, storage cost, and accuracy). We first try to report the numbers in the original papers for each decision factor. We then design several empirical studies in case the papers do not evaluate certain decision factors.

% To this end, we systematically studied XX \ac{pedr} systems published in top security, system, and AI conferences in 20XX - 20XX. These approaches include five rule-based systems and eight learning-based systems. We summarize the general description of these systems in Table~\ref{tab:compare}. For these 13 research papers, we investigate whether they have been evaluated against the seven decision factors. We list their reported values of the seven decision factors in Table~\ref{tab:literature}. The empty cells mean the corresponding paper does not evaluate the corresponding decision factor.

% \textbf{General Gap.} In general, we notice that most papers focus on evaluating the accuracy of detection. All of them fail to evaluate at least one must-meet decision factor mentioned by the industrial experts. This study shows that there is a huge gap between the industry and the academia in the understanding of \ac{pedr} systems. 


% In this section, we analysis the characteristic of different models and their performance according to the data from their paper. Then we present the results of our experiments on several classic models. We describe our experiment setup and the datasets. Then we show the performance of these models and compared with the requirements in industrial deployment.

\eat{
\begin{tcolorbox}[title=Gap 1, left=2pt, right=2pt, top=2pt, bottom=2pt]
Academia needs to pay more attention to \textsf{Client-Side Overhead}, which is the most important decision factor for adopting \ac{pedr} systems.
\end{tcolorbox}
}
% . For instance, as shown in , there are no evaluations on the client-side overhead for Auditd, Sysdig, LTTng, and ETW, which are . Other provenance collectors in Table~\ref{tab:collectors} only evaluates the runtime overhead of their approach, but overlook the memory consumption. 
% Furthermore, their evaluations may not be comprehensive by only evaluating the client-side overhead with one high-end hardware configuration. For instance, Quicklog was evaluated on a machine with 18 cores~\cite{quicklogger}. In this case, the evaluation may be biased. 



%  This indicates that we need to better optimize the efficiency of existing provenance collectors to meet the expectations of the industry.

\eat{
Even worse, we find that existing provenance collectors may underestimate their runtime overhead by only evaluating with high-end machines. As shown in Table~\ref{tab:benchmarkidle}, provenance collectors tend to slow down the monitored hosts more on machines with fewer cores. For instance, Auditd can slow down Nginx by 597\% on a physical machine with 1 CPU core while it only slows down Nginx by 10.90\% on a virtual machine with 32 CPU cores. We can observe similar patterns for Sysdig and LTTng.  This is because these three provenance collectors, including their variants (Quicklog, KennyLoggings, Hardlog), adopt a single-threaded architecture. This architecture limits the CPU usage of the provenance collector by only allowing one collector thread running.  Therefore, the runtime overhead on a machine with many CPU cores could be lower since the provenance collectors can, at most, take one CPU core. Unfortunately, we notice that low-end machines with less than two CPU cores are still popular today.  According to a report~\cite{awsanalysis}, more than 40\% instances on AWS are micro or small instances, which have 1-2 CPU cores. Thus, overlooking low-end machines may harm the usefulness of provenance collectors.

For memory consumption, we find no evaluation in the papers in Table~\ref{tab:literature} or in the provenance collectors in Table~\ref{tab:collectors}. This indicates a general neglect of memory consumption in existing work. According to the results from our measurement study in Table~\ref{tab:collectormem}, Sysdig consumes too much memory for machines with many CPU cores since it allocates 8MB memory for each CPU core.

Auditd and LTTng also need to be more memory efficient. According to our experiment result in Table~\ref{tab:collectormem}, they consume 65.9MB and 79.9MB memory on machines with 32 CPU cores, respectively.  
Although these numbers seem just to satisfy the reference value (< 100MB, according to Table~\ref{tab:QualitativeResult}), they may still be too high in practice. Remember that in our experiment in Section~\ref{sec:measurementclientside}, we took a minimalist approach in our experiment. We have only keep the most basic logic of each provenance collector. However, in practice, \ac{pedr} systems may need to add extra compression and pre-processing logic to provenance collectors that may consume more memory that exceed the expectation of engineers. 
}





% \noindent\textbf{Client-side Overhead:} For performance loss, according to the data listed in Table~\ref{tab:collectors} and evaluated in Table~\ref{tab:benchmarkidle}, we can find that most of the average application performance losses are higher than the requirement of industry. Particularly, the performance loss is highly correlated with the types of applications. It has a greater drawback on the performance of io-intensive applications, while have little performance loss on computing-intensive applications. In addition, the performance loss is related to hardware configuration. This is determined by the design of the collectors. For example, current collectors limit the CPU usage of the collector by only allowing \textit{one collector thread.} in order to minimize the system run-time overhead. Therefore, on a machine with more cores, there will be less resource competitions between the collector and the application, resulting in a less decrease in the performance of the application.


% For memory consumption, we find neither industrial nor academic collectors have systematically evaluated memory consumption. Most of the collectors need to configure the size of kernel buffer for caching the log entries. However, it is usually neglected by the users and they just use the default configurations in the simplest way. In our experiment, the memory consumption is also related to hardware configuration. For example, Sysdig and Lttng follows the per-CPU buffering scheme. As the total number of CPU cores increases, the memory consumption continues to increase.   

% In conclusion, the overhead of client-side collector must be taken seriously in academic research and industrial development. Thus, we propose the guideline of how to evaluate the overhead of collectors. (where to add the finding "small number of cpu cores are more popular")
\eat{
\noindent\textbf{Gap 2: Alarm Triage vs. Precision}
The second gap between the industry and the academia is how they evaluate the effectiveness of a \ac{pedr} system in reducing false positives. 
While academic papers use precision to measure how effectively a \ac{pedr} system reduces false positives, the managers prefer the alarm triage cost, measured by the average number of alarms generated per host per day. 

As shown in Table~\ref{tab:InterviewResult}, only two managers consider precision as an optional decision factor for them. 
This does not imply that precision is not important, but rather indicate that it is not straightforward to estimate labor cost using precision.
The reason is that in practice, the ratio between the number of attacks and the number of system audit events is extremely low, and thus the number of reported alarms per day per host can be high even if the precision is high ($>0.9$). 


the number of attacks 


precision depends on the number of true positives (\ie attacks), which varies across datasets.

convert precision into labor cost. 
As discussed in Section~\ref{sec:rq2}, the key bottleneck for the industry to adopt a \ac{pedr} system is the comprehensive cost. 
However, it is difficult to calculate how much labor cost is required to triage false alarms solely based the precision. The reasons is that precision depends on the number of true positives, which varies across datasets. Thus, the managers can hardly have a stable estimation to the man-hour needed to triage alarms in practice.

The average number of alarms per host per day, on the flip-side, is a good complementary factor for precision. On the one hand, on a dataset with few attacks, the average number of alarms is defacto the number of false positives. Thus, it can reflect the ability of a \ac{pedr} system when attacks are rare. On the other hand, it is straightforward for a manager to estimate how many man-hour he needs to process the alarms of a \ac{pedr} system, as the processing capability of a security engineer is a fixed number. In this case, the manager can convert the alarm triage cost as a part of the comprehensive cost when adopting a \ac{pedr} system. 


\eat{
First of all, precision, although designed to reflects the false positive rate, is not a good indicator of a \ac{pedr} system's ability to avoid false positives when attacks are extremely rare. Remember that $precision=\frac{TP}{TP+FP}$, where $TP$, $FP$ are the numbers of true positives and false positives, respectively. This metric could be significantly affected by the ratio of attacks in a dataset. 

Let's consider an extreme dataset that contains no attacks. On this dataset, any \ac{pedr} systems cannot yield true positives. Thus, the precision will always be zero. In this case, precision is useless. Unfortunately, in practice, datasets with few attacks are common. Therefore, the industrial managers do not consider precision as an important decision factor, according to Table~\ref{tab:InterviewResult}.
}




\begin{tcolorbox}[title=Gap 2, left=2pt, right=2pt, top=2pt, bottom=2pt]
    \textsf{Alarm Triage}, measured by the average number of alarms per host per day, is a necessary complementary metric for precision.
    \end{tcolorbox}
% Third, recall is not observable in practice. In realistic settings, the number of false negatives cannot not be accurately measured due to the colossal number of events. Thus, according to the managers we have interviewed, a common practice in the industry is to measure the recall of an \ac{pedr} on a testing dataset. As long as the recall number is higher than a threshold, people considers the \ac{pedr} can effectively detect attacks. 
}

% By carefully examining these systems, we notice that caching all the provenance data in the memory is a catastrophic design. 
% As shown in Table~\ref{tab:memcost}, the larger the provenance graph, the more memory HOLMES and ProveDetector consume. 
% These two systems cache all the provenance data in the memory so that they cannot support large cluster monitoring, 

% \eat{
% \begin{tcolorbox}[title=Gap 4, left=2pt, right=2pt, top=2pt, bottom=2pt]
% Researchers and developers need to raise enough attention on memory consumption and prevent reserving too much provenance data in memory.
% \end{tcolorbox}
% }
% According to our study, the average memory consumption of \ac{pedr} di\noindent\textbf{Server-side Overhead:} d not attract enough attention and there is a large gap in server-side memory consumption between academia and industry. In an industrial environment, \ac{pedr} is deployed on a detection server for the intrusion detection of the cluster. Therefore, the memory consumption is determined by the amount of provenance data collected from each monitored client, which means that the average memory consumption cannot be neglected. It determines how we configure the server to be capable of monitoring the whole cluster. 

% However, our study finds that most of the existing \ac{pedr} cannot meet the industrial requirements, allocating 30 - 40 MB of memory on average to each client. In our evaluation in Section~\ref{sec:computing}, the memory consumed by HOLMES and ProvDetector is positively correlated with the data volume of the provenance graph, which both exceed the requirements by 1-2 orders of magnitude. For UNICORN, it has relatively stable memory consumption, which is preferred in an industrial environment, because it uses Parallel Sliding Windows (PSW) algorithm to analyze the whole provenance graph independent of memory constraints. However, it also exceeds the requirement. But it provides a feasible way to use memory under constraints.


% \noindent\textbf{alarm Triage and Investigation Cost:}
% alarm triage cost and investigation cost are neglected by academia, but very crucial indicators in the industry. Existing \ac{pedr} systems in academia cannot meet these two requirements at the same time, so that the detection results cannot be responded in time within the analysts' processing capabilities, thus facing the problem of alarm fatigue. 

% Table~\ref{tab:literature} shows that all the \ac{pedr} systems in academia do not take triage cost and investigation cost into consideration because the cluster size in academia evaluations is too small, merely several clients. However, the real cluster size in the industry is generally more than 1000 clients. Table~\ref{tab:alarm-number} and Table~\ref{tab:graph-size} shows that HOLMES, ProvDetector and UNICORN can not meet the requirements at the same time. Although the size of detected provenance graph of HOLMES and ProvDetector are controlled at the hundredth level, the average alarm numbers far exceed the industiral requirements, listed in Table~\ref{tab:QualitativeResult}. The average number of alarms in unicorn roughly meets the target, whereas the graph size is around 100,000, far exceeding the requirements.


\eat{
alarm triage cost和investigation cost是被学术界忽略，但是在工业界十分重要的指标。学术界P-EDR系统无法同时满足两个指标，其告警结果无法在分析师的处理能力范围内被及时响应，因而面临告警疲劳问题。
表格x中学术界所有的P-EDR系统都忽略triage cost，主要原因在于实验主机的规模，学术界的实验主机仅有在1-2台，而工业界真实数据集普遍在1000台终端以上。表格11和12measurement实验结果显示，三个系统均无法没有同时满足两个指标。holmes与provdetector虽然graph size控制在100左右，但是average alarm number远超指标值。unicorn的平均告警数量虽然大致满足指标，但是graph size在十万左右，远超指标值。
}













% \eat{
% \subsection{Machine Cost: Client-side Overhead}
% % \usepackage{multirow}
% % \usepackage{booktabs}

% % \begin{table}
% % \centering
% % \caption{List of existing provenance data collectors}
% % \label{tab:collectors}
% % \resizebox{0.49\textwidth}{!}{\begin{tabular}{ccccc} 
% % \toprule
% %                & Platform & Owner                    & Affect & Community  \\ 
% % \midrule
% % Sysdig~\cite{sysdig}         & Linux    & Sysdig.Inc               &        & Industry   \\
% % Linux Audit~\cite{auditd}    & Linux    & Linux Foundation         &        & Industry   \\
% % Camflow~\cite{camflow}        & Linux    & University of Cambridge  &        & Academia    \\
% % LTTng~\cite{fournier2009combined,desnoyers2008lttng}          & Linux    & EfficiOS                 &        & Industry   \\
% % ETW ~\cite{etw}           & ~Windows & Microsoft                &        & Industry   \\
% % KennyLoggings~\cite{paccagnella2020logging} & Linux    & UIUC                     &        & Academia    \\
% % Hardlog~\cite{ahmad2022hardlog}        & Linux    & Microsoft                &        & Academia    \\
% % Quicklog~\cite{281386}       & Linux    & Florida State University &        & Academia    \\
% % \bottomrule
% % \end{tabular}}
% % \end{table}


% % Table\ref{tab:compare} lists the comparison of \ac{ids} models that emerged in recent five years, from 2017 to 2022. They can be divided into two categories: \textbf{rule-based} and \textbf{learning-based}. Rule-based models are designed to utilize human prior knowledge to match the kill chain or propagate the information on the provenance graph, such as HOLMES, POIROT, SLEUTH, and MORSE. The learning-based models learn the behaviors from history data without using human prior knowledge and detect the anomalies in path-level or graph-level, such as Log2vec, ProvDetector, UNICORN and SHADEWATCHER. As we can see, most of the models are closed source, expect for UNICORN and SHADEWATCHER. Therefore we choose to re-implement HOLMES and ProvDetector, setup UNICORN and SHADEWATCHER using the public source code to evaluate them on our datasets. Then we analysis other models according to the data list in their paper.

% \subsection{Machine Cost: Server-side Computing Cost}
% \label{sec:computing}
% According to our interviews with industrial experts, the server-side computing cost, measured by the average memory cost per monitored host, is the second must-meet requirement for machine cost. Therefore, in this section, we investigate whether existing \ac{pedr} systems meet this requirement. 

% To this end, we combine literature and empirical measurement studies. We first investigate the reported server-side memory consumption of \ac{pedr} systems and list the results in Table~\ref{tab:literature}. The values are either directly reported in the papers or estimated by dividing the total memory consumption by the number of hosts in the corresponding dataset. Then, for those approaches that do not evaluate server-side cost in their paper, we try to implement them and measure their server-side cost with open and industrial datasets. 

% \subsubsection{Empirical Measurement}
% We choose to implement ProvDetector~\cite{}, UNICORN~\cite{}, and HOLMES~\cite{} to empirically evaluate their server-side memory cost. We cannot implement RapSheet~\cite{} because it relies on unpublished rules from security companies. We also omit the investigation systems like PrioTracker, NoDoze, ATLAS, and DEPCOMM because they need to work with unpublished third-party attack detection tools.  
% -

% We use five datasets to evaluate the server-side computing cost of ProvDetector, UNICORN, and HOLMES. Among the three datasets, DARPA-CADETS, DARPA-THEIA, and DARPA-TRACE are open datasets from DARPA. REAL CUSTOMER is the dataset of customers of a security company \anosec. SIMULATION is an in-lab dataset we created for attack simulation. We list the high-level information of these datasets in Table~\ref{tab:memcost}


% Particularly, CADETS contains three attacks during a three-day-long period. The attacker exploited the vulnerabilities of an Nginx server and achieved C\&C by injecting the payload to an ``sshd'' process. The attacker repeated the attack three times. He failed the first two times but succeeded in the last one.
% THEIA has one attack. The attacker first exploited the Firefox backdoor to install executable files to disk. After two days, he used the vulnerability of a browser extension and resumed the prior attack by injecting the file that had been previously dropped to disk into the ``sshd'' process.
% TRACE has two attacks, the first one is a Firefox backdoor with the DRAKON malware in memory, and the second one is a Pine backdoor with a DRAKON dropper.


% REAL CUSTOMER was collected by {\anosec}'s EDR deployed in the customers' network, which includes 300+ servers and working machines of employees of 10 industrial customers from \anosec, including schools, research institutes, factories, and healthcare providers. We monitor the customers for five days. We use the first three days (training period) to train the detection model,  and use the last two days (test period) for testing.


%  The SIMULATION dataset was collected from five hosts: one Ubuntu 20.04 server (U1), two Windows Server 2012 R2 Datacenters (S1,S2), one Windows Server 2019 Datacenter (S3),  and one Windows 10 desktop host (D1). We deployed Apache and PostgreSQL on Windows Servers and Nginx and PostgraSQL on Ubuntu 20.04 to simulate servers in the \anosec. We used the Windows ten desktop to simulate the PCs used by the employees in the \anosec. The collected data have the same format as Sysdig for Linux and ETW for Windows. 

 
% \begin{table}[t]
%     \centering
%     \caption{Overview of the evaluation datasets}
%     \resizebox{0.48\textwidth}{!}{
%     \begin{tabular}{|c|c|c|c|c|c|c|}
%     \hline
%     \multirow{2}{*}{Dataset} & Host &\multirow{2}{*}{Days}& Data & Event & Event & Event\\
%     &Num & & Size&Num & Rate & Size \\\hline
%     DARPA-CADETS & 1 & 11 & 14 GB & 15 M& 16.87 eps &1013 Byte \\ \hline
%     DARPA-THEIA & 1 & 11 & 7.5 GB& 10 M& 11.25 eps &810 Byte\\ \hline
%     DARPA-TRACE & 1 & 11 & 62 GB&  72 M& 75.76 eps & 925 Byte\\ \hline
%     SIMULATION & 5 & 12 & 23 GB & 50 M &  48.23 eps& 483 Byte\\\hline
%     REAL CUSTOMER & 300+ & 5 & 16.85 GB & 17M &  39.35 eps& 1064 Byte\\\hline
%     \end{tabular}}
%     \label{tab:ground-truth}
% \end{table}


% We show the experiment results in Table~\ref{tab:memcost}. We notice overall, the reported values of existing \ac{pedr} systems can meet the expectations of industrial experts, which is 30-40MB memory per host. However, we also notice that approaches, such as Poirot and ZePro fail to meet this requirement. Therefore, we conclude that the memory consumption on the server side for different \ac{pedr} systems varies. People need to carefully optimize server-side memory consumption to meet the expectations of industrial experts.


% \begin{tcolorbox}[title=Server-side Computing Cost, left=2pt, right=2pt, top=2pt, bottom=2pt]
% We find that existing provenance collectors are generally satisfying in server-side computing cost. However, a \ac{pedr} still need to carefully optimize the memory consumption on the server side to meet the expectation of industrial experts. 
% \end{tcolorbox}
% \begin{table}[t]
%     \scriptsize
%     \centering
%     \caption{Memory Cost}
%     \begin{tabular}{|c|c | c c c|}
%     \hline
%     \multirow{2}*{\textbf{Dataset}} &  \textbf{\#Average} & \multicolumn{3}{c|}{\textbf{Server-side Computing Cost (MB/host)}} \\ \cline{3-5}
%     & \textbf{Graph Nodes} & HOLMES  & ProvDetector & UNICORN\\ \hline  
%     DARPA-CADETS & 280W+ &   5.55G  & 10G & 274M     \\\hline
%     DARPA-THEIA & 125W+ &  3.78G & 6.42G &  242M    \\ \hline
%     DARPA-TRACE & 325W+    & 9.38G & - &  242M      \\ \hline
%     In-lab Arena &  3W+ &     73M & 195M & 213M     \\ \hline
%     Real Customer  &   5W+   & 84M & 240M & 219M.   \\ \hline
%     \end{tabular}
%     \label{tab:memcost}
% \end{table}
% \subsection{Labor Cost: alarm Triage Cost}
% Industrial experts rank the alarm triage cost as the second most important decision factor. Thus, in this section, we investigate whether existing provenance analysis techniques can meet the expectations of industrial experts.

% Unfortunately, our investigation shows that none of the existing approaches evaluate the key metric for the alarm triage cost, which is the average number of alarms per monitored host. Indeed, existing approaches fail to put the accuracy of an \ac{pedr} in the context of cost. Thus, they only evaluate the accuracy alone. 

% To this end, we make a measurement study with the three \ac{pedr} systems we implemented in Section~\ref{sec:computing}. Note that although we only implemented three \ac{pedr} systems, they are representative. First, these three systems have the highest precision according to Table~\ref{tab:literature}. Since the average number of alarms approximates the precision (See Section~\ref{sec:laborcost}), we expect these three systems to have the lowest number of alarms per host per day. Second, these three systems cover the two categories of \ac{pedr} systems. HOLMES is one of the state-of-the-art rule-based systems, while UNICORN and ProvDetector are the two leading learning-based systems. We measure the number of alarms per host per day for these three \ac{pedr} systems with the same datasets used in Section~\ref{sec:computing} and list the results in Table~\ref{tab:alarm-number}.

% \begin{table}[!t]
%     \scriptsize
%     \centering
%     \caption{Average alarm Number(/host/day)}
%     \begin{tabular}{|c|c|c|c|}
%     \hline
%     \textbf{Dataset} &\textbf{ HOLMES} &\textbf{ProvDetector} &  \textbf{UNICORN} \\ \hline
%     DARPA-CADETS    & 21 & 90 & 0.3                        \\ \hline
%     DARPA-THEIA &    36.7 & 90 & 0.1                     \\ \hline
%     DARPA-TRACE   & 13.9 & - & 0.45                       \\ \hline
%     In-lab Arena  & 2.3 & 23 & 0.09                     \\ \hline
%     Real Customer & 12.1  & 56.3 & 0.13                         \\ \hline
%     \end{tabular}
%     \label{tab:alarm-number}
% \end{table}

% Our experiment shows that only UNICORN can roughly meet the expectations of the experts(<0.1 alarms/host/day). HOLMES and ProvDetector still need to reduce the number of alarms by magnitudes to meet the expectations of experts from the industry. Specifically, since precision determines the number of alarms per host per day (See Section~\ref{sec:laborcost}), HOLMES and ProvDetector still need to improve their precision significantly.

% \begin{tcolorbox}[title=alarm Triage Cost, left=2pt, right=2pt, top=2pt, bottom=2pt]
% Most \ac{pedr} systems still need to reduce the number of alarms per monitored host per day by magnitudes to meet the expectation of industrial experts. 
% \end{tcolorbox}

% \subsection{Labor Cost: Investigation Cost}
% \dingli{I will merge 7.3 and 7.4 later}
% Investigation cost, measured by the size of generated provenance graphs, is the fourth must-meet requirement of \ac{pedr} systems, according to our interviews in Section~\ref{sec:interview}. Therefore, we investigate whether existing \ac{pedr} systems can meet the requirement of investigation cost.

% To this end, we first investigate the reported graph size in literature and also make a measurement study on the three \ac{pedr} systems we implemented in Section~\ref{sec:computing}. We report the result of the investigation in Table~\ref{tab:literature} and the  measurement study in Table~\ref{tab:graph-size}.

% \begin{table}[t]
%     \scriptsize
%     \centering
%     \caption{Average Graph Size}
%     \begin{tabular}{|c|c|c|c|}
%     \hline
%     \textbf{Dataset} &\textbf{ HOLMES} &\textbf{ProvDetector} &  \textbf{UNICORN} \\ \hline
%     DARPA-CADETS    &     173 & 15 & 154730                        \\ \hline
%     DARPA-THEIA &    73 & 8 & 522735                     \\ \hline
%     DARPA-TRACE   & 450 & - & 1454033                       \\ \hline
%     In-lab Arena  &     566 & 7 & 11587                     \\ \hline
%     Real Customer   & 81 & 5 & 17853                         \\ \hline
%     \end{tabular}
%     \label{tab:graph-size}
% \end{table}

% Interestingly, we observe that existing \ac{edr} systems fail to balance the investigation cost and the triage cost.
% For the \ac{edr} systems that meet the experts' expectations of investigation cost (<10-100 nodes in provenance graphs), they fail to achieve satisfying triage cost. For instance, in Table~\ref{tab:literature}, MORSE and RapSheet can roughly meet the requirement of investigation cost. However, their precision is lower than 0.5, indicating a high number of alarms per host per day in practice. In Table~\ref{tab:graph-size}, HOLMES and ProvDetecor also have concise provenance graphs that meet the expectations of experts. Yet, these two approaches need to reduce the number of alarms by magnitudes. On the flip side, the triage cost of UNICORN is satisfying. However, UNICORN generates too coarse-grained provenance graphs that are three to four magnitude larger than the expectations of experts. 

% With more investigations, we find there is a trade-off between the investigation cost and the triage cost. Assume that the volume of provenance data is fixed. Generating larger provenance graphs can reduce the total number of alarms, leading to fewer number of alarms per host per day. For instance, assume a monitored host generates 10M nodes in a single huge provenance graph. A coarse-grained \ac{pedr} system, such as UNICORN, only generates one alarm that covers the whole provenance graph. Thus, its average number of alarms per host per day is low. On the contrary, fine-grained approaches, such as ProvDetecor, generates hundreds of alarms, each covering a subset of the whole provenance graph. Therefore, fine-grained approaches have a higher triage cost. Overall, we identify how to balance the triage cost and investigation cost as a challenge for provenance techniques. 

% % \begin{tcolorbox}[title=Investigation Cost, left=2pt, right=2pt, top=2pt, bottom=2pt]
% % Existing \ac{pedr} systems need to balance the investigation cost and triage cost better. 
% % \end{tcolorbox}
% % \dingli{I don't think our current data makes the network and storage cost interesting. I suggest removing these two points. Yet, we can discuss}
% % \subsection{Experiment Setup}
% % \subsubsection{Environment}

% \section{Summary of Our Study(Suggestions for Future Study)}
% \begin{itemize}
%     \item Reduce the client-side overhead, optimize collectors
%     \item Balance Triage Cost and Investigation Cost
% \end{itemize}
% % Many \ac{ids} models have emerged over the past few years, and they can be divided into two categories: rule-based and learning-based. Rule-based models are designed to utilize human prior knowledge to match the kill chain or propagate the anomaly score on the provenance graph. HOLMES is the state-of-the-art rule-based real-time \ac{ids}. It uses 16 rules concluded from hundreds of APT reports~\cite{} and Common Attack
% % Pattern Enumeration and Classification (CAPEC) defined by US-CERT and DHS with the collaboration of MITRE~\cite{}. Based on these rules, HOLMES matches the low-level system events to high-level attack stages.  The learning-based models learn the behaviors from history data without using human prior knowledge and detect the anomalies in path-level or graph-level. ProvDetector is a typical learning-based model to detect stealthy malware in path-level. It reports the rarest paths of provenance graph as malicious. UNICORN is the first system to detect intrusions via runtime analysis of naive whole-system provenance, which means its detection is graph-level. It computes a fixed-size graph sketch as the graph growing and clusters the sketch to detect whether the graph is anomaly. Based on the above characteristic, as shown in Table\ref{tab:compare}, these three models can represent the \ac{ids} in detection methods and detection results. 

% % Therefore, in our experiments, we choose three provenance-based models, HOLMES, UNICORN, and ProvDetector, to evaluate the performance of the pain points. We implemented it according to the 16 rules listed in the paper. We configured the blacklist of suspicious IPs and sensitive programs on the labeled ground truth. Furthermore, we fine-tuned the parameters for HOLMES to achieve the best accuracy for each dataset, respectively. As for UNICORN, we directly used the published source code of UNICORN, but modified its data parser to accept our data format. We implemented ProvDetector xxx.



% \subsection{Dataset}
% We evaluate these models on six public and commercial datasets, including three public datasets: CADETS, THEIA, and TRACE from DARPA TC, an industrial internal security evaluation dataset (Industrial Arena), a simulated attack dataset (In-lab Arena), and a historical attack detection dataset for two customers (Real Customer) from AnonymousSec. The Industrial Arena dataset contains the data of an internal security daily monitoring of \anosec, which consists of 14-day provenance data from 1,130 hosts (168 Windows hosts and 962 Linux). The In-lab Arena dataset is created by us to simulate some well-known \ac{apt} attacks and the attacks that have occurred in \anosec. The In-lab Arena dataset is publicly available at \url{https://xxx}. The Real Customer dataset is the historical data of two customers of \anosec, which contains provenance data of xxx Windows hosts. Table \ref{tab:ground-truth} shows the summary of these datasets. We discuss the details of the datasets as follows.



% \noindent\textbf{CADETS, THEIA, TRACE:} The three public datasets are from DARPA TC \ac{e3} program. We choose not to use \ac{e5} because it misses several documented critical attack steps in the logs such that we cannot reconstruct the attack campaigns manually.
% CADETS contains three attacks during a three-day-long period. The attacker exploited the vulnerabilities of an Nginx server and achieved C\&C by injecting the payload to an ``sshd'' process. The attacker repeated the attack three times. He failed the first two times but succeeded in the last one.
% THEIA has one attack. The attacker first exploited the Firefox backdoor to install executable files to disk. After two days, he used the vulnerability of a browser extension and resumed the prior attack by injecting the file that had been previously dropped to disk into the ``sshd'' process.
% TRACE has two attacks, the first one is a Firefox backdoor with the DRAKON malware in memory, and the second one is a Pine backdoor with a DRAKON dropper. 

% \noindent\textbf{Industrial Arena Dataset:}
% We built the Industrial Arena dataset by collecting provenance data from {\anosec}'s Security Operations Center (SoC), using the internal \ac{edr}. The dataset includes the provenance logs of a 14-day internal daily monitoring. The SoC monitored 1,130 hosts (168 Windows hosts and 962 Linux) in the company and collected the provenance data in a centralized virtual machine (16 CPUs, 32GB RAM, and 1TB hard disk) running 64bit CentOS 7.4. During the 14-day long collection, the system auditing logs collected in the hosts contain $\sim$1.6 billion system events (1.63TB) in total. The experts of the security team analyzed the alarms that were triggered by commercial \ac{edr}, but no attack was found. So this dataset is supposed to be pure.

% \noindent\textbf{In-lab Arena Dataset:}
% Besides the Industrial Arena dataset, we also built a smaller testbed that simulated the internal environment of the \anosec and made the collected data publicly available. The data were collected from five hosts: one Ubuntu 20.04 server (U1), two Windows Server 2012 R2 Datacenters (S1,S2), one Windows Server 2019 Datacenter (S3),  and one Windows 10 desktop host (D1). We deployed Apache and PostgreSQL on Windows Servers and Nginx and PostgraSQL on Ubuntu 20.04 to simulate servers in the \anosec. We used the Windows ten desktop to simulate the PCs used by the employees in the \anosec. The collected data have the same format as Sysdig for Linux and ETW for Windows.  

% We conducted seven different attacks, including well-known \ac{apt} attack: APT29, FIN6, SideWinder, four real attacks occurred in the \anosec. On S1 and U1, we carried out two real attacks from \anosec. The attacker exploits the Apache Struts2-046 (CVE-2017-5638) vulnerability~\cite{struts2-046} for remote code execution and then penetrates the database on U1 by exploiting weak passwords. And on S1, the attacker exploits the ``phpstudy'' backdoor and uses ``PAExec.exe'' to control other Windows servers remotely. We also simulated two data stealing campaigns that happened in \anosec on S2 and D1. On S2, employee A stole employee B's account password, logged into B's host, searched for some useful confidential files, collected, packaged and transferred them to personal accounts through cloud disks. During the second attack, the \ac{apt} compromised the D1 and move laterally to S2 and stole the important data on it. On D1, we also carried out APT29~\cite{apt29}, FIN6~\cite{FIN6} and SideWinder~\cite{SideWinder} using the Atomic Red Team~\cite{atomictest} and techniques based on MITRE's ATT\&CK~\cite{mitre}.  


% \noindent\textbf{Real Customer Dataset:}
% Our sixth dataset is the historical data of seven real customer of \anosec. The data of this dataset were collected by the EDR deployed in the customer's network, which includes 300+ servers and working machines of employees of 10 industrial customers from \anosec, including schools, research institutes, factories, and healthcare providers. We monitor the customers for five days. We use the first three days (training period) to train the detection model,  and use the last two days (test period) for testing.

% % \begin{itemize}
% %     \item Public dataset: 3 + 2
% %     \item sangfor dataset: 2
% %     \item real world: 2 customers
% %     \item DARPA: E3 cadets, theia, trace
% % \end{itemize}
% % \subsection{Model Performance}
% % In this section, we conduct the experiments to evaluate the performance of these three models on the pain points that are concluded from the survey. First, we calculate the overall cost of deploying the \ac{edr} in the industry for daily monitoring. Second, we evaluate the quality of the alarms, including the number of alarms and the number of false positives and the granularity.

% % \noindent\textbf{Cost:} In the survey, operational cost is the most critical factor in whether the \ac{edr} can be deployed within the enterprise. For centralized \ac{edr}, it mainly consists of four aspects: Memory, CPU, Network and Storage. So we evaluate the overall cost of the three models from these four aspects. 

% % \begin{itemize}
% %     \item \textbf{CPU}: 
% %     \item \textbf{Storage}:
% %     \item \textbf{Network}:
% %     \item \textbf{Memory}:
% % \end{itemize}

% % \begin{table*}[t!]
% %     \scriptsize
% %     \centering
% %     \caption{Memory Cost.}
% %     \begin{tabular}{|c|c|c |c|c|c |c | c c c|}
% %     \hline
% %     \multirow{2}*{\textbf{Dataset}} & \multirow{2}*{\textbf{Host Type}} &\multirow{2}*{\textbf{\#Host}}  & \multirow{2}*{\textbf{\#Campaigns}} & \multirow{2}*{\textbf{Duration}} & \multirow{2}*{\textbf{\#Events}} & \multirow{2}*{\textbf{\#Average Graph Nodes}} & \multicolumn{3}{c|}{\textbf{Average Memory Cost}} \\ \cline{8-10}
    
% %     & & & & & & & HOLMES  & ProvDetector & UNICORN\\ \hline  
% %     DARPA-CADETS                      & Linux        &   1     & 3                                       &      10d                     &15M+                           & 280W+ &   5.55G & 10G & 274M                           \\ 
% %     \hline
% %     DARPA-THEIA                      & Linux        &   1    & 1                                       &      10d                     &10M+                           & 125W+ &  3.78G & 6.42G &  242M                      \\ 
% %     \hline
% %     DARPA-TRACE                      & Linux         &  1    & 2                                       &     11d                      &72M+                           & 325W+    & 9.38G & - &  242M                       \\ 
% %     \hline
% %     In-lab Arena                   & Linux + Windows  &       5       & 7                               &    7d                        & 36M+                          &  3W+ &     73M & 195M & 213M                     \\ \hline
% %     Real Customer        & Windows                     &  2  &      1                                   &      8d                     &     3M+                           &   5W+   & 84M & 240M & 219M                            \\ \hline
% %     \end{tabular}
% %     \label{tab:ground-truth}
% % \end{table*}

% \begin{table}[t]
%     \scriptsize
%     \centering
%     \caption{Memory Cost}
%     \begin{tabular}{|c|c | c c c|}
%     \hline
%     \multirow{2}*{\textbf{Dataset}} &  \textbf{\#Average} & \multicolumn{3}{c|}{\textbf{Server-side Computing Cost (MB/host)}} \\ \cline{3-5}
%     & \textbf{Graph Nodes} & HOLMES  & ProvDetector & UNICORN\\ \hline  
%     DARPA-CADETS & 280W+ &   5.55G  & 10G & 274M     \\\hline
%     DARPA-THEIA & 125W+ &  3.78G & 6.42G &  242M    \\ \hline
%     DARPA-TRACE & 325W+    & 9.38G & - &  242M      \\ \hline
%     In-lab Arena &  3W+ &     73M & 195M & 213M     \\ \hline
%     Real Customer  &   5W+   & 84M & 240M & 219M.   \\ \hline
%     \end{tabular}
%     \label{tab:memcost}
% \end{table}

% % \noindent\textbf{alarm Quality:}
% % The quality of alarms also greatly effects the detection efficiency. 





% % \begin{itemize}
% %     \item HOLMES: rule-based, real-time, event-level
% %     \item UNICORN: learning-based, real-time, graph-level
% %     \item ProvDetector: learning-based, offline, event-level
% % \end{itemize}

% % metric: 
% % \begin{itemize}
% %     \item RQ1: memory, cpu time, disk, GPU, throughput(online or offline)
% %     \item RQ2: alarm rate, false positive
% %     \item RQ3: graph size, granularity, can pinpoint attack nodes?
% % \end{itemize}
% % \subsection{Result Analysis}
% % \noindent\textbf{Domain Reason of Cost:}

% % \noindent\textbf{Balance in alarm Quality:}
% % \subsection{Gap 1: Network Cost}

% % \subsection{Gap 2: Storage Cost}
% % \subsection{Gap 3: Runtime Cost}
% % \subsection{Gap 4: Alarm Quality}
% % \subsection{Gap 5: Investigation Cost}
% % \subsection{Gap 6: Senmantic Gap}

% \subsection{Gap in Machine Cost}
% \begin{table}[t]
%     \centering
%     \caption{Cost comparison between different models}
%     \resizebox{0.48\textwidth}{!}{
%     \begin{tabular}{|c|c|c|c|c|}
%     \hline
%     \textbf{Model} & \textbf{$Cost_N$} & \textbf{$Cost_S$} & \textbf{$Cost_C$} & \textbf{Host Cost} \\\hline
%     \multirow{2}{*}{HOLMES} & \multirow{6}{*}{\shortstack{2.58GB/day/host\\(0.31USD)}} & \multirow{6}{*}{\shortstack{2.58GB/day/host\\(0.25USD)}} & \multirow{2}{*}{\shortstack{6.24GB\\(52.7USD)}} & \multirow{2}{*}{53.26USD}\\
%     & & & & \\ \cline{1-1}\cline{4-5}
%     \multirow{2}{*}{ProvDetector} & ~ & ~ &\multirow{2}{*}{\shortstack{8.1GB\\(68.4USD)}}  & \multirow{2}{*}{68.96USD}  \\
%     & & & & \\ \cline{1-1}\cline{4-5}
%     \multirow{2}{*}{UNICORN} & ~ & ~ & \multirow{2}{*}{\shortstack{252.67MB\\(2.1USD)}} & \multirow{2}{*}{2.66USD} \\ 
%     & & & & \\ \hline
%     \end{tabular}}
%     \label{tab:cost}
% \end{table}

% In the survey, machine cost is the most critical factor in whether the \ac{edr} can be deployed within the enterprise. We have summarized four key decision factors of machine cost through our survey: \textit{Client-side Overhead, Network, Storage and Computing}. Existing \ac{pedr}s are centralized so that the client-side overhead is mainly coming from provenance data collection, which is out of the scope of our experiments. So we evaluate the other three factors in the followings.
% % \begin{equation}
% %     HostCost = Cost_N*\alpha_n + Cost_S*\alpha_s + Cost_C*\alpha_c
% % \end{equation}
% % where $Cost_N$, $Cost_S$ and $Cost_C$ denote the network bandwidth, the average storage size and the average memory usage of per host, and $\alpha_n$, $\alpha_s$, $\alpha_c$ denote the price parameters of network bandwidth, storage and memory respectively. Specifically, $Cost_N$ is calculated using the average number of transmissions per host per second. $Cost_S$ is calculated  using the average amount of raw data generated by a host in one day.  $Cost_C$ is calculated using the average memory footprint during the detection procedure in the server. For price parameters, we calculate according to market price~\cite{}. 

% \noindent \textbf{Network Cost ($Cost_N$).}
% For CADETS, THEIA and TRACE dat aset, they are collected from their respective single host. They must transmit the auditing data generated in real-time to the server for detection in time. Therefore, the minimum bandwidth needs to meet the real-time transmission of the collected logs to the detection server. So we can calculate the requirement of average network bandwidth using the data transfer rate per second, which is 2.58GB/day/host for DARPA cluster.

% \noindent \textbf{Storage Cost ($Cost_S$).}
% For all these three models, $Cost_S$ is mainly brought about by storing raw data generated during daily system auditing. In other words, it is the size of raw data stored on the hard disk. The DARPA dataset that we used in our experiments is about 83.5GB of data on three hosts for about 10-11 days. Therefore the average $Cost_S$ is 2.58GB/day/host. It is the same as the $Cost_N$ because all the data in DARPA dataset is required to transmit to the detection server and store on the disk. 

% \noindent \textbf{Computational Cost ($Cost_C$).}
% We measure the memory usages using the footprints of these three models. We record the footprints of memory consumption every one second. Figure\ref{fig:memory} shows the footprint of memory usage. In our experiment, the average memory usages of HOLMES, ProvDectector and UNICORN are 6.24G, 8.1G and 257.67MB respectively. For HOLMES and ProvDetector, the memory consumption grows quickly in data loading and graph building procedures because they maintain almost all the data in the memory and never evict it out. For UNICORN, it extracts the graph into a fixed-size graph sketch, periodically cleans up subgraphs in memory and keeps only the extracted sketches. Therefore the memory consumption of unicorn is maintained at a relatively stable level. However, the memory consumption is highly correlated with the size of the sketch. In its paper, with sketch size 10,000, memory consumption increases up to 2.5GB.




% Compared to the requirements in the survey, we find that the gaps in network, storage and memory are all unacceptable to commercial products. The amount of logs collected and uploaded on the client side to the server greatly affects the $Cost_N$ and $Cost_S$. It is desirable to transmit only 50MB auditing logs and store only 200MB per host per day. However, the raw data collected on a host are two orders of magnitude higher than the requirements. Therefore there is a large gap in network transmission and storage between industry and literature.



% The computational cost is the largest gap due to retention of provenance data in memory. Table\ref{tab:cost} shows that the overall cost of per host is unacceptable expensive for industry provenance analysis. We calculate according to market price~\cite{}. Among these three factors, we can find that these models are about the same on $Cost_N$ and $Cost_S$, both of which are much less than $Cost_S$, which means that $Cost_C$ accounts for the majority of cost. Therefore, the \textit{\textbf{computational cost} is the most concerned in system provenance analysis deployment}. In our study, the industry expect 50MB per host, however, existing techniques consume 5GB memory on average. Therefore they cannot meet the requirement of the industry. 



% Table\ref{tab:memcost} shows that the huge provenance graphs cached in the memory are the root cause of computing overhead and the reasons for the huge size of provenance graphs in memory are two folds. First, there are a lot of redundancy in the provenance data. As the Table\ref{tab:ground-truth} shows, DARPA, the most widely used public dataset, has a large amount of data and the event generation rate is extremely high on the three different hosts. In our experiments, we find that there are a lot of redundancy events in the raw data. For example, xxxx. So it can puts huge pressure on provenance graph construction and memory consumption. However, existing technique fail to address these redundancies. Second, existing techniques consume more and more memory when provenance data grows. Figure XXX shows the growth of memory usage as the provenance data consuming. However, since provenance analysis techniques are expected run 24/7 for months to detect APT attacks, such a memory consuming pattern is not good. 





% Therefore, we suggest three possible directions to improve existing techniques. First, we need to develop techniques that reduce redundancies in provenance data. Second, we need to design methods that can eventually remove unimportant provenance data from the memory to keep a constant memory consumption. Third, we can take a distributed approach to detection and monitoring. To have a preliminary result on the effectiveness of these two directions, we developed a simple redundancy reduction technique and a simple method that removes unimportant provenance data from the memory.

% Our redundancy deduction method has XXX steps. First, XXXX, second XXXX. After using this simple redundancy reduction method, we reduce the memory usage of current techniques by xxx\% while still keeping the similar accuracy (or only losses XX\% accuracy). Table/Figure XXX shows this result. This preliminary result shows that redundancy reduction could substantially reduce the memory cost of provenance analysis while keep the accuracy.

% Our method that removes provenance data from memory does XXX, XXX and XXX. After using this method, we can keep the memory usage at a constant. Table/Figure XXX shows this result. We can see that the accuracy does not decrease too much by keeping the memory constant.





% \subsection{Gap in Labor Cost}
% % \textbf{Existing tools cannot meet the requirements for alarming}
% % \begin{itemize}
% %     \item Accuracy rate is not stable in large scale cluster. The high accuracy rate fine-tuned on certain datasets cannot be extended to other datasets.
% %     \item Accuracy rate neglect other properties.
% %     \item The labor cost is the fundamental factor that we should consider when deploying \ac{edr} in the industrial environment.
% %     \item So we introduce the metric of alarm quality
% % \end{itemize}
% In our survey, we find that labor cost is also key factors in deploying commercial \ac{edr} in enterprises environments. In this section, we evaluate the labor cost of exisiting models from two aspects: interpretation cost and alarm triage cost, instead of using accuracy rate. 

% For common sense, accuracy rate is an important metric to evaluate the performance of the \ac{edr}. As shown in Table\ref{tab:compare}, existing tools have achieved an extremely high accuracy rate, however they cannot be adopted into the industrial environment. For commercial \ac{edr}, it is comprehensible that the higher the accuracy, the better. However, focusing on improving accuracy cannot meet the industrial requirements.


% On the one hand, the high accuracy rate is unstable in large scale cluster. The fact is that there are lots of false alarms in large scale monitoring. However, the attack activities are rare compared to the normal behaviors. So the number of alarms will increase substantially as the size of the cluster grows, requiring a corresponding increase in human labor to handle these alarms. For example, Figure\ref{} shows the growth trend of the number of alarms with the number of machines in our cluster.


% % \begin{table}[t!]
% %     \centering
% %     \caption{Accuracy rate}
% %      \resizebox{0.48\textwidth}{!}{
% %     \begin{tabular}{|c| c  c | c  c | c  c |}
% %     \hline
% %     \multirow{2}*{\textbf{Dataset}} &
% %     \multicolumn{2}{c|}{\textbf{HOLEMS}} & \multicolumn{2}{c|}{\textbf{ProvDetector}} & \multicolumn{2}{c|}{\textbf{UNICORN}}  \\  \cline{2-7}
% %     & \textbf{Precision} & \textbf{Recall}& \textbf{Precision} & \textbf{Recall} & \textbf{Precision} & \textbf{Recall} \\ \hline
% %     % \multicolumn{1}{|l|}{Dataset} & \multicolumn{1}{l|}{Host Type} & \multicolumn{1}{l|}{\#Campaigns} & \multicolumn{1}{l|}{Duration} & \multicolumn{1}{l|}{\#Events} & \multicolumn{1}{l|}{\#Actions} \\ \hline
% %     DARPA-CADETS            & 1.00 &  1.00 & 0.03 & 1.00 & 1.00 & 1.00                 \\ 
% %     \hline
% %     DARPA-THEIA         & 1.00 &   1.00 & 1.00 & 1.00 & 1.00 & 1.00                           \\ 
% %     \hline
% %     DARPA-TRACE      & 0.28&  1.00 & 0.15 & 1.00 & 0.67& 1.00                            \\ 
% %     \hline
% %     Industrial Arena  & 0.67 & 1.00 & 0.04  & 1.00 & 1.00 & 1.00                         \\ \hline
% %     In-lab Arena      & 0.50 & 1.00 & 0.04 & 1.00 &1.00 &1.00                         \\ \hline
% %     Real Customer   & 0.33 &1.00 &NA & NA& 1.00& 1.00                                  \\ \hline
% %     \end{tabular}
% %     }
% %     \label{tab:accuracy}
% % \end{table}


% % On the other hand, focusing on only the accuracy rate can neglect other properties that are important in attack detection and investigation. When deploying \ac{edr} in an industrial environment, we must consider the labor costs of monitoring and alarm analysis, which cannot be fully reflected by accuracy rate. 

% On the other hand, accuracy rate cannot reflect the alarm fatigue problem that the industry often encounters. We define alarm fatigue problem as \textit{the number of nodes that are reported is far more than the security analysts can handle}. In our survey, security analyzers suffer from alarm fatigue for a long time. 


% \eat{大规模集群不稳定}
% Therefore, we evaluate the labor cost from interpretation cost and alarm triage cost, which can directly reflect the practicability and efficiency on provenance analysis. It mainly consists of two aspect: (1) \textbf{the amount of alarms} and (2) \textbf{the analyzability of each alarms}. We find that there is a certain contradiction between these two metirc. We evaluate the alarm quality of the models on xxx datasets. We configure each model on each dataset to achieve the best performance, which is the best accuracy, as shown in TableXXX. Then we analysis the quality of alarms as follows.

% \textit{The amount of alarms is still unacceptable for the analyzers to handle the situation}. Table\ref{tab:alarm-number} shows the alarm number of these models on different dataset. Our study shows that in an industry, each analyzer monitors XXX machines on average and can deal with XXX-XXX alarms in a day. However, our experiment shows that only UNICORN can satisfy this requirement. 

% \begin{table}[!t]
%     \scriptsize
%     \centering
%     \caption{Average alarm Number(/host/day)}
%     \begin{tabular}{|c|c|c|c|}
%     \hline
%     \textbf{Dataset} &\textbf{ HOLMES} &\textbf{ProvDetector} &  \textbf{UNICORN} \\ \hline
%     DARPA-CADETS    & 21 & 90 & 0.3                        \\ \hline
%     DARPA-THEIA &    36.7 & 90 & 0.1                     \\ \hline
%     DARPA-TRACE   & 13.9 & - & 0.45                       \\ \hline
%     In-lab Arena  & 2.3 & 23 & 0.09                     \\ \hline
%     Real Customer & 12.1  & 56.3 & 0.13                         \\ \hline
%     \end{tabular}
%     \label{tab:alarm-number}
% \end{table}

% \textit{The analyzability of each alarms is also important for attack detection and reconstruction}. Most of the existing models report subgraphs for the analyzers as an alarm. However, the size of the subgraphs directly affects the analyzability of alarms.  Table\ref{tab:graph-size} shows the results of our experiment on the average graph size of each alarm. We find two crucial problems from the results: (1) \textbf{coarse-grained alarms} and (2) \textbf{fragmented alarms}. For UNICORN, it reports the whole provenance graph as an alarm, which is so huge that the analyzer cannot locate the root cause of the attack. For ProvDetector, although the analyzer can check whether an alarm is related to attacks with high efficiency, they will spend much more time connecting the suspicious alarms to reconstruct the whole attack scenario to understand the attack. In our survey, the analyzers prefer the size of alarms between XXX and XXX. However, most of the models cannot satisfy this requirement. 

% Table\ref{tab:alarm-quality} summarizes whether existing models can satisfy the above two requirements. We can find that there is no models can satisfy both two requirement of alarm quality in industry. Therefore, we suggest that we need to find a balance in the above two requirements. To achieve the desirable object, we have two suggestions. 
% First, we can merge the similar alarms or combine the related alarms to reduce the amount of alarms and merge the similar nodes/events in the detected results. 
% Second, we need to find balance in detection granularity. To avoid coarse-grained and fragmented detection, we need to provide enough guidance, such as the most suspicious processes or the critical paths, in the subgraph that can contain the whole attack campaign.




% \subsection{Gap in Senmantic}\label{sec:SenmanticGap}


% \begin{table}[t]
% \centering
% \caption{The alarm quality of different models}
% \label{tab:alarm-quality}
% \begin{tabular}{c|c|c}
% % \toprule

%              & Amount of alarms  &  Size of alarms \\ 
% \hline
% SLEUTH~\cite{} & \Circle  & \CIRCLE  \\ 
% Poirot~\cite{} & \CIRCLE & \Circle \\
% HOLMES~\cite{milajerdi2019holmes}  & \LEFTcircle     & \LEFTcircle \\
% % SWIFT~\cite{} &  & \\
% MORSE~\cite{} & \Circle &  \LEFTcircle \\
% ProvDetector~\cite{wang2020provdetector} &  \Circle        & \Circle     \\
% UNICORN~\cite{han2020unicorn}      & \CIRCLE      & \Circle  \\ 
% WATSON~\cite{} & \Circle   & \LEFTcircle  \\
% SHADEWATCHER~\cite{} &  \Circle & \CIRCLE \\ 
% \hline
% \end{tabular}
% \end{table}

% In our survey, we find that the style for alarm representation is also highly concerned by security team. There are many research on bridging the semantic gap between low-level system logs and high-level attack behavior, such as the provenance graph summarization~\cite{} and behavior abstraction~\cite{}. However, xxx\% of interviewees think that the original provenance graph is enough for attack investigation and automatic semantic abstraction based on expert knowledge is not necessary. There are two reasons that will be discussed as follows.

% On the one hand, analyzers can get detail and complete information from the original provenance graph. Provenance graph is used to visualize system activities and help people better understand the connection between system events. The concise and small provenance graph is good enough for the analyzers to find out the attack campaign. Semantic abstraction can help analyzers annotate the attack steps sometimes. However, the performance of existing models is not stable enough for daily analysis. For example, xxxxx. It can always mislead the analyzers and add extra analysis overhead.



% On the other hand, existing tools for semantic abstraction cannot meet the requirements of being applied in industry provenance analysis. In our survey, we also interviewed the experienced security experts what is the ideal style for alarm representation. As shown in Figure\ref{XXX}, XXXXX. However, to achieve the ideal representation, existing tools face two serious challenges. First, we need to find a comprehensive and concise way for expert knowledge extraction and formal representation. Prior expert knowledge is indispensable in high-level semantic abstraction and it is mainly gotten from CTI reports and the description of the attacks in MITRE. So the quality of knowledge extraction determines the performance of semantic abstraction. Second, the final representation needs to provide relatively crucial low-level information, such as the filename of malicious script, the abnormal process, and the malicious IP address. In this way, the analyzers can find out the procedure of the attack in detail and take appropriate action, such as deleting the crucial files and killing the process.


% \eat{
% 1、graph-based 成本高
% 2、成本高- 内存占用
% 3、大部分方法都需要建图，graph size -> memory
% 4、两个数据集上差异较大，采集方式；精度，语意抽象。
% }

% \eat{
% cost结论，引出研究方向：怎么减少计算成本
% 1. 分布式
% 2. 检测可以由局部到整体，避免整体建图
% 3. 

% 告警消减：
% 1. 很重要，可能需要组合式方法
% 2. rank排序，告警排序
% 3. 大家这些方法都不太够把告警压缩下来


% 语义gap：
% 1. 不需要语义抽象也可以进行分析
% 2. 分析员最终需要什么样的语义信息（最终希望得到每一步攻击是怎么做的）
% 3. 现有的有什么问题（1. rule-based model需要先验知识，无法防范未知的攻击 2.距离最终希望得到的表示还有一定距离 ）
% }

% \eat{
% 1. 现有工具尽可能多分析几个，说清楚为什么选这么几个，可以用论文上的实验数据。
% 2. 
% }

